Reinforcement Learning for Dynamic Resource Allocation in Optical Networks: Hype or Hope?

The application of reinforcement learning (RL) to dynamic resource allocation in optical networks has been the focus of intense research activity in recent years, with almost 100 peer-reviewed papers. We present a review of progress in the field, and identify significant gaps in benchmarking practices and reproducibility. To determine the strongest benchmark algorithms, we systematically evaluate several heuristics across diverse network topologies. We find that path count and sort criteria for path selection significantly affect the benchmark performance. We meticulously recreate the problems from five landmark papers and apply the improved benchmarks. Our comparisons demonstrate that simple heuristics consistently match or outperform the published RL solutions, often with an order of magnitude lower blocking probability. Furthermore, we present empirical lower bounds on network blocking using a novel defragmentation-based method, revealing that potential improvements over the benchmark heuristics are limited to 19-36% increased traffic load for the same blocking performance in our examples. We make our simulation framework and results publicly available to promote reproducible research and standardized evaluation https://doi.org/10.5281/zenodo.12594495.

==> 2_PAPER_SECTIONS/1_introduction.tex <==
\section{Introduction}

% Is the motivation for applying RL to increase capacity or to increase uatoation? Both! But more so dynamicity and automation.

Network operators are faced with a problem: how to increase capacity for fast-growing data traffic without increasing the price of services \cite{lord_future_2021}. Advances in transmission technology have so far provided the solution by exponentially increasing the point-to-point capacity of the optical channel. However, as the throughput of the installed C+L bands approaches the nonlinearity-limited information bounds \cite{shtaif_information_2024}, costly infrastructure upgrades are required to scale capacity through spatial division multiplexing or ultra-wideband transmission \cite{winzer_future_2023}. Operators seek to minimize or delay the required capital expenditure and offset it with reduced operational costs. Online optimization of network resource allocation offers a path towards these aims by increasing the achievable network throughput with dynamic and automated service provisioning. 

Reinforcement learning (RL) has emerged as a promising technique for dynamic resource allocation (DRA) from a range of exact solution methods, heuristic algorithms, and artificial intelligence (AI) approaches.  RL solutions can approach the quality of exact methods such as integer linear programming (ILP), with an online allocation time comparable to simple heuristics \cite{di_cicco_deep_2022}. In fact, many works have demonstrated RL solutions that are superior to selected heuristics across various optical network problems %\cite{chen_deeprmsa_2019,chen_multi-task-learning-based_2021,xu_deep_2022} 
 (see section \ref{sec:survey}).

However, despite the many papers that investigate RL for optical networks, adoption of machine learning (ML) techniques by network operators has been limited by non-technological barriers \cite{khan_non-technological_2024}. One barrier is a lack of clear benchmarks and demonstrable benefits. Studies of resource allocation problems in optical networks often present results on specific topologies and traffic models, without fair comparison to previous results. Often results are not generalizable. 

In this paper we address this barrier by providing analysis of and recommendations for benchmarking practices. We identify 5 papers that provide the best examples of benchmarking in the field and exactly recreate their problem settings. By "problem settings", we mean the exact network topologies, traffic models, and other details of the network simulations. We then evaluate a range of heuristic algorithms and apply the best to each case. The best heuristic algorithms outperform or equal the reported RL results in all cases.

To understand if it is possible to improve on these new benchmarks, we propose a heuristic-based lower bound network blocking estimation method, termed Resource-Prioritized Defragmentation (section \ref{sec:bounds}). For each case of study, we apply this method over a range of traffic loads and estimate that the supported traffic load at a fixed blocking (0.1\%) may be increased by 19-36\% for flex-grid networks. These estimates suggest further improvement is possible.

This is the first time that a thorough analysis and benchmarking of previous work has been carried out, and highlights deficient benchmarking standards. Our findings suggest that previous attempts to find better resource allocation policies using RL have been unsuccessful, and new efforts are required to find solutions, using RL or other methods, that improve on the best benchmarks and approach the estimated bounds.

%We also investigate the limits of network throughput for dynamic traffic, to understand how much additional data traffic could be supported by improved resource allocation. We propose a heuristic-based lower bound network blocking estimation method, termed Resource-Prioritized Defragmentation (section \ref{sec:bounds}). For each case of study, we apply this method over a range of traffic loads and estimate that the supported traffic load at a fixed blocking (0.1\%) may be increased by 19-36\% for flex-grid networks. These estimates may motivate further research on optimized DRA with RL or other methods.

This paper aims to: 1) Promote higher standards for evaluation and benchmarking in research on RL for DRA. 2) Improve reproducibility and transparency of research by open sourcing our simulation framework and providing discussion of implementation details that significantly affect results (e.g. path ordering in Section 4.\ref{sec:path_ordering} and holding time truncation in Section 5.\ref{sec:holding_time}). 3) Encourage new research into optimized DRA by demonstrating that previous RL approaches have failed to beat our benchmarks but there remains a considerable optimality gap between the benchmarks and our estimated bounds.

The contributions of this work are:
\begin{enumerate}[itemsep=0pt]
    \item A comprehensive survey of progress on RL approaches to DRA in optical networks.
    \item A systematic study of the factors affecting heuristic algorithm performance and recommendations for the best heuristic benchmarks.
    \item A recreation of problems from five landmark papers in the field with comparisons to improved heuristic benchmarks, showing previous RL results have failed to improve on heuristics.
    \item The introduction of a novel empirical throughput bound estimation method, which shows benchmarks are not near-optimal.
    \item The release of our simulation framework, "XLRON", to promote reproducible research and enable fair comparison across different studies.
\end{enumerate}

All of the code necessary to generate data and plots from this paper are available on Github \cite{michael_doherty_micdohxlron_2024}.

We begin with essential background on DRA problems and RL techniques in Section 2, followed by a literature review in Section 3. Section 4 presents the investigation of heuristic algorithms for benchmarking. Section 5 details the analysis of the previously published results and comparison with benchmarks. Section 6 presents new empirical bounds for network throughput, with recommendations for future research directions in Section 7.






% These results have important implications for the optical networks research community. 
% Firstly, the need for good benchmarking practices is highlighted. Secondly, the relative performance of RL is shown to be overstated. Finally, the benefits of RL for the DRA problems analyzed in this paper are limited. Overall, this implies the community needs to improve its benchmarking practices and foster a culture of open source to help ensure that future research results are not spurious, and shift focus to problems with a sufficient optimality gap for which there do not exist already-strong heuristics.

% The contributions of this paper are:
% \begin{enumerate}
%     \item The first comprehensive survey of RL applied to DRA problems in optical networks.
%     \item Reproduction of previously published results with thorough benchmarks, that show RL performance to be inferior to simple heuristics.
%     \item New estimates of network capacity upper bounds show improvement over the best-performing heuristics is limited to 1-36\%.
%     \item We make publicly available "XLRON", our Python simulation library used to produce all results in this paper, for other researchers \cite{doherty_xlron_2023}.
% \end{enumerate}

% All of the code necessary to generate data and plots are available here \cite{michael_doherty_micdohxlron_2024}.

% %The overall contribution of the combined survey, reappraisal, and upper-bound estimation, is to provide guidance to the research community on fruitful future research directions. The performance of previous RL solutions, based on blocking probability, is surpassed by simple heuristics, therefore demonstrating superior RL performance remains an outstanding problem. However, the performance ceiling is estimated to already be close (XX-XX\%) for simple algorithms, which may prompt researchers to pursue other avenues to boost network throughput and efficiency.


% \noindent The rest of this paper is structured as follows. Section \ref{sec:background} provides the background required to understand DRA problems and RL techniques. Section \ref{sec:survey} discusses the papers reviewed and how they were selected. The reviewed works are categorized for discussion according to their contributions. Section \ref{sec:repro} focuses on 5 influential papers from the literature and our work to recreate their cases of study in simulation. We benchmark heuristics to determine the best one in each case, we describe and quantify implementation details for each case of study, and we present the results from benchmarking previous work. We then describe our empirical network capacity bound estimation method and present our estimates of the gap between our upper bound estimates and best performing heuristics. Finally, conclusions are drawn in Section \ref{sec:conclusion}.



% uggestions from Claude:
% Network operators face mounting pressure to increase capacity for ever-growing data traffic while maintaining constant service prices \cite{lord_future_2021}. While advances in transmission technology have historically met this challenge through exponential increases in fiber optic channel capacity, the approach of the non-linear Shannon limit for C+L bands \cite{shtaif_information_2024} now necessitates costly infrastructure upgrades \cite{winzer_future_2023}. Operators therefore seek to optimize their existing infrastructure through better resource allocation methods.
% Reinforcement learning (RL) has emerged as a heavily researched approach for dynamic resource allocation (DRA) in optical networks, offering solutions that match the quality of exact methods like integer linear programming while maintaining the fast allocation of simple heuristics. The field appears well-suited for RL given its large search space, clear optimization objectives, and ability to generate training data through simulation \cite{hassabis_nobel_2024}. This has led to numerous papers claiming superior performance over traditional methods.
% However, we identify critical issues in how this research has been conducted and evaluated. Through a comprehensive review of the literature and reproduction of results from five influential papers, we demonstrate that properly tuned heuristic algorithms consistently match or outperform the published RL approaches. Furthermore, using a novel defragmentation-based method, we establish theoretical upper bounds showing that potential improvements over current heuristics are limited to just 1-36% increased capacity.
% Our findings have profound implications for the field:

% The advantages of RL for these problems have been significantly overstated due to inadequate benchmarking
% Many supposed advances may be artifacts of poor experimental methodology
% The limited room for improvement suggests research efforts may be better directed elsewhere

% The key contributions of this work are:

% The first comprehensive survey and critical analysis of RL approaches to optical network DRA
% A unified simulation framework enabling fair comparison across different studies
% Rigorous reproduction of key results showing the superiority of simple heuristics
% Novel theoretical bounds quantifying the limited potential for improvement
% Release of our XLRON simulation library to promote reproducible research

% This paper aims to reset expectations in the field and establish higher standards for evaluation and reproducibility in optical networking research. We begin with essential background on DRA problems and RL techniques in Section 2, followed by our literature analysis in Section 3. Section 4 presents our detailed reproduction of previous results and new theoretical bounds. We conclude with recommendations for future research directions in Section 5.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Maybe keep the mention of SDN, dynamic operation, EON and low-margin operation for the background section. The emerging paradigms of software defined networking (SDN) and dynamic operation open a path to automated... EONS allow low-margin ioperation


% 60% of operating costs are from field and service operations (McKinsey report) but tbh that refers to call centre and customer support operations seemingly.


%The resource allocation problems that are presented by optical networks fall under the category of combinatorial optimisation, for which a range of exact and approximate solution methods exist \cite{bengio_machine_2020}. Artificial intelligence techniques, specifically the use of deep reinforcement learning (DRL), are a more recent candidate to solve these problems, as they offer faster online execution than linear programming methods and potentially superior optimisation performance than heuristic algorithms.


% Next I want to make the point that P2P capacity has increased exponentially and is widely considered to have approached the non-linear Shannon limit. Therefore optimistion of resource allocation to traffic flows becoming increasingly attractive. Dynamic operation, in which traffic flows are serviced on-demand, precludes the option of exact solution methods with exorbitant calculation times.  Previously ILP was able to find exact solution (can also cite Meta paper from ONDM). 
%Advances in DSP, coherent transceivers, amplifiers, ROADMs and other network components have allowed traffic  to increase 
%Consequently, increasingly sophisticated techniques have been proposed to efficiently allocate bandwidth on optical fibres to connect geographic sites. This problem, of routing and resource allocation, occurs in systems ranging from metro to inter-data centre, national and continental scale networks. % cite handbook of optcal networks? or a review paper

%The majority of published works focus on dynamic traffic, with small numbers for static and incremental traffic.

% dynamic, static, incremental
%Connection requests are static (known a priori), dynamic (stochastic arrival and departure), or incremental (stochastic arrival and no departure). 


%Useful review paper of RWA, RSA, RCSA \cite{zhang_overview_2020}


% \subsection*{Scope of work}
% For completeness, we include works that focus on both fixed-grid and flex-grid 



% Firstly, the need for good benchmarking practices is highlighted. A lack of standardization in problem settings and open source code has made it difficult to compare to previous approaches. This has allowed insufficient benchmarking practices to propagate in the literature. By thoroughly benchmarking against the best performing heuristics, RL fails to improve on heuristics in nearly all cases shown. The community therefore needs to adopt better practices to ensure future published results are not spurious.

% Secondly, the benefits of RL for the DRA problems analysed in this paper are limited. Our empirical upper bounds on network capacity suggest that the focus should be shifted to problems where the optimality gap of current heuristics is significant enough to merit the application of RL. Joint optimisation tasks, e.g. of SNR and network throughput, for which heuristics are not readily available, could be a more fruitful area.

%We identify the various problem settings that have been examined (including network topologies, available bandwidth, and traffic models) and the algorithms against which RL solutions have been benchmarked. 

%To test the robustness of the reported performance of RL solutions against common benchmark algorithms, we select 5 prominent papers from the literature 
% maybe provide motivation for the selected papers here
%\cite{chen_deeprmsa_2019,shimoda_mask_2021,tang_heuristic_2022,xu_deep_2022,cheng_ptrnet-rsa_2024} and recreate their cases of study. We first reproduce the reported results in each paper for the K-shortest paths first-fit (KSP-FF) heuristic, then compare with the published figures. As a product of this comparison, we identify implementation details that materially affect the results and quantify their impact. These details we refer to as network traffic warmup period (the amount of traffic used to pre-populate the network prior to training or evaluation) and the ordering of the pre-calculated shortest paths used by heuristics. By taking account of these details and optimising the path ordering, we demonstrate that simple heuristics outperform the reported RL results in all of the works we examine.

%To complete the analysis of examined problems, we estimate the upper-bound performance for each case of study with 2 techniques: 1) cut-set analysis \cite{cruzado_capacity-bound_2024} and 2) ordered request assignation. Cut-sets analysis relaxes constraints to provide a loose upper bound, while ordered request assignation provides a tighter bound. Together, the upper bounds show that the possible improvements in supported traffic levels for the cases of study are only XX-XX\%.


==> 2_PAPER_SECTIONS/2_background.tex <==
% Background contains technical details necessary to understand the work

% First subsection covers resource allocation and routing umbrella term (mention how this differentiates between routing on a network with scalar capcity vs vector, and also that the definition excludes multicast/NFV/VONE. We focus on unicast with link resources (no node resource considerations)), then RWA, RSA, RMSA.

\section{Background}
\label{sec:background}


\subsection{DRA problems in optical networks}

%\subsubsection*{Network Capacity and Low-Margin Operation}
%The optical data communication infrastructure that underpins metro, inter-data center, national and continental scale networks presents a range of optimization problems. The objective of these problems is to maximize the network throughput (the sum of realized point-to-point data transmission connections) within the constraints of available resources, most crucially the available bandwidth on links.

%The complexity of these systems has grown as networks have become increasingly flexible in the parameters of each transmitted channel; including launch power, symbol rate, modulation format and channel spacing. This flexibility is enabled by now-ubiquitous coherent transponders with advanced DSP, and ROADMs that support varying spectrum granularity. The highly configurable nature of each channel opens opportunities to increase network utilization through low-margin operation \cite{auge_can_2013}. Unallocated margins and system margins \cite{pointurier_design_2017} can be reduced with this technology by matching the requested and available channel capacity and reach, and mitigating non-linear effects through launch power allocation, respectively. Moving from fixed-grid (50GHz or greater channel spacing) to flex-grid (minimum 6.25GHz channel) spacing allows more precise matching of requested data transmission capacity to bandwidth. Network capacity is further enhanced by judicious allocation of routes and bandwidth to network traffic, which is the primary task of DRA problems.

\subsubsection*{Motivation for dynamic operation and RL}
As discussed by Aug\'e \cite{auge_can_2013} and Pointurier \cite{pointurier_design_2017}, optical networks must operate with a margin of additional resources between the minimum requirements to fulfill a data service request and the resources allocated to that request, for example by allocating additional spectrum. This margin is required due to uncertainty in physical parameters of the transmission network or future traffic variations. Reducing the margin can increase the network throughput or reduce costs.

Dynamic operation allows the allocated resources to vary temporally in response to shifting traffic, thereby allowing more accurate matching of resources to current demand, which reduces margins. The time constraints of dynamic operation may preclude exact solution methods, but a trained RL agent can compute an allocation in sub-second time \cite{di_cicco_deep_2022}.

RL is appropriate for these problems because they possess three characteristics that merit the application of AI \cite{hassabis_nobel_2024}: 1) a large combinatorial search space, 2) a clear objective function for optimization, and 3) plentiful training data and/or accurate and efficient simulators for data generation. 
%\cite{nevin_techniques_2022,di_cicco_deep_2022}.

\subsubsection*{Traffic models}
Network traffic comprises a set of requests to connect source and destination nodes with fixed data rates on dedicated lightpaths. Traffic can be modeled as static, incremental, or dynamic \cite{zang_review_2000}.

Static traffic assumes knowledge of all connection requests that the network must accommodate. Incremental traffic lies between static and dynamic in stochasticity: requests are not known in advance but do not expire once allocated. For dynamic traffic, connection requests are served on-demand without knowledge of future requests, and active connections expire randomly. The request arrival and expiry times are sampled from probability distributions, often assumed to be exponential \cite{chen_deeprmsa_2019}. Dynamic traffic is considered a paradigm for future optical networks, that have the necessary systems in place to enable real-time response to changing network conditions \cite{lord_flexible_2022}.

%In current production networks, traffic demand is typically forecast for a given period e.g. one year, and resources allocated and configured in advance. Additional unforecast demand may then be added incrementally. Dynamic traffic is therefore a paradigm for future optical networks, that have all the necessary software and hardware systems in place to enable real-time response to changing network conditions  \cite{lord_flexible_2022}.
%In this paper, we consider only dynamic traffic, as this paradigm offers the , though we note that previous research into wavelength-routed networks found dynamic operation only increased total capacity in networks with wavelength conversion capability \cite{zapata-beghelli_dynamic_2008}.

%The traffic model spatial characteristics are defined by the traffic matrix. %In dynamic or incremental settings, the traffic matrix elements are normalized probabilities of a connection between the nodes corresponding to the column and row indices \cite{nevin_techniques_2022}. %In static settings, a traffic matrix element may represent the total data rate between the node pair \cite{jaumard_decomposition_2023}. %It is common practice to consider uniform traffic matrices for DRA problems.

\subsubsection*{Problem variants}
The classic optimization problem in an optical network is Routing and Wavelength Assignment (RWA) for fixed-grid networks or Routing and Spectrum Assignment (RSA) for flex-grid networks, where spectrum is divided into frequency slot units (FSU) \cite{mukherjee_springer_2020}. Further degrees of freedom in the optimization are added by considering the selection of \underline{M}odulation formats (R\underline{M}SA), and the fiber \underline{C}ore or spectral transmission \underline{B}and utilized by each channel in the case of multi-core or multi-band networks (R\underline{C}MSA/R\underline{B}MSA). Launch \underline{P}ower has also been considered as a parameter in the optimization objective for dynamic networks (R\underline{P}MSA) \cite{ives_routing_2015} \cite{arpanaei_launch_2023}.% and is a relatively under-investigated problem variant.  

While most DRA problems in optical networks from the literature are concerned with point-to-point connections, some consider virtual networking tasks such as virtual optical network embedding (VONE) \cite{gong_virtual_2014,doherty_deep_2023} or virtual network function placement (VNF) \cite{zhou_applications_2022}. We choose to focus on RWA/RSA/RMSA in this paper because they are the most widely studied DRA problems in the context of optical networks and they form a core sub-task of variants such as VNF or VONE.

% Overview paper of problem types (also inlcudes details on ML/RL but very limited and with poor understanding): \cite{zhang_overview_2020}


\subsubsection*{Constraints}
Three fundamental constraints govern resource allocation in optical networks:
%transparent\footnotemark optical networks:

%\footnotetext{This assumes lightpaths are routed "transparently" at nodes without optoelectronic conversion for the purposes of signal regeneration or wavelength conversion.}

\begin{enumerate}[itemsep=0pt]
    \item Spectrum Continuity: A lightpath must use identical FSU on each link, without wavelength conversion.
    \item Spectrum Contiguity: FSU allocated to a lightpath must be adjacent.
    \item No Reconfiguration: Active lightpaths cannot be reallocated once established, meaning allocation decisions are permanent while connections remain active.
\end{enumerate}

The 'No Reconfiguration' constraint is not a physical limitation but an operational assumption that active services cannot be disrupted. Reconfiguration may sometimes be desirable, especially in flex-grid networks that may suffer from spectral fragmentation \cite{gerstel_elastic_2012}, and has been used in a production network by Meta Platforms Inc. to free up spectral resources \cite{balasubramanian_targeted_2023}.



\subsubsection*{Solution methods}
%The possible methods to solve the DRA problems depend on whether the traffic is static or dynamic. Static traffic allows analytical approaches for exact combinatorial optimization, most notably Integer Linear Programming (ILP). ILP formulations have been suggested for DRA problems \cite{walkowiak_ilp_2016}, but the application of ILP to realistic problem sizes of networks with capacity for thousands of connection requests remains computationally infeasible \cite{jaumard_decomposition_2023}.% The RWA problem for static traffic has been shown to be NP-hard \cite{chlamtac_lightpath_1992}. Consequently, the computational complexity scales super-polynomially with the topology size and traffic load for RWA and related problems.


Allocation of static traffic is a NP-hard combinatorial optimization problem \cite{chlamtac_lightpath_1992}, for which the computational complexity of finding a solution scales super-polynomially with the space of possible allocations. Exact solution methods such as Integer Linear Programming (ILP) have been formulated for static traffic \cite{walkowiak_ilp_2016,jaumard_decomposition_2023} but show limited scalability\footnotemark and are infeasible for dynamic traffic without a priori knowledge of all requests. \footnotetext{\cite{jaumard_decomposition_2023} Jaumard et al. scale their ILP formulation to 690 requests on the USNET topology (24 nodes and 86 links) with 380 FSU per link, without considering distance-adaptive modulation formats.}

For dynamic traffic, any allocation decision must be taken within the constraint of the time interval between request arrivals. No standard limit has been defined for this constraint in the literature but it could be on the order of seconds, with a lower limit set by the switching time of reconfigurable optical add-drop multiplexers (currently 1ms to 100ms, depending on the switching technology \cite{goto_lcos-based_2024}).

Many simple heuristic algorithms \cite{vincent_scalable_2019,abkenar_best_2016,wright_minimum-_2015,tang_heuristic_2022,savory_congestion_2014} have been proposed for these problems, with the goal to minimize resources, lightpath distances and required bandwidth. Heuristics have the advantages of fast execution time and deterministic and interpretable allocation decisions.

Machine learning approaches to DRA problems have included nature-inspired techniques like particle swarm optimization (PSO) \cite{hassan_chaotic_2009} and genetic algorithms (GA) \cite{barpanda_genetic_2011}. Once trained, an RL policy can compute an allocation faster than other ML approaches \cite{di_cicco_deep_2022}.

\subsection{Reinforcement learning}
\label{sec:background_rl}

RL is a framework for learning to optimize sequential decision making under uncertainty. It emerged from Bellman's foundational work on optimal control theory in the 1950s, specifically dynamic programming and Markov Decision Processes (MDP) \cite{bellman_theory_1954,bellman_markovian_1957}. MDPs model decision-making processes as an agent that takes actions in an environment to maximize a reward signal. The method of action selection is a mapping from states to actions termed the policy, which can be expressed in tabular form or approximated by a neural network (NN). The use of NN for function approximation is sometimes distinguished as "Deep" RL. Tabular RL has been applied to optical networks \cite{terki_routing_2023}, but function approximation with NN is widely used \cite{chen_deeprmsa_2019,shimoda_mask_2021,tang_heuristic_2022,xu_deep_2022,cheng_ptrnet-rsa_2024} when the set of state-action pairs is too large to be tabulated \cite{sutton_reinforcement_2018}.

The reader is referred to Sutton and Barto's authoritative textbook \cite{sutton_reinforcement_2018} for details. However, to aid the discussion of RL applied to DRA problems, several terms are defined here.

RL algorithms can be classified as model-based or model-free. Model-based RL uses a model of the environment to plan future actions, but so far no works have applied this paradigm to DRA problems in optical networks. Model-free RL algorithms learn through direct interaction with the environment, without planning. Model-free algorithms can be further categorized into:
\begin{itemize}
\item \textbf{Action-value methods}, such as Q-learning, which learn to estimate the value of taking actions in different environment states. These methods were the first to be developed in RL \cite{watkins_learning_1989,sutton_learning_1988} and have been used for route selection in optical networks \cite{bryant_q-learning_2022}.
\item \textbf{Policy gradient methods}, which directly optimize the policy parameters to maximize expected rewards. These methods can handle continuous action spaces, unlike action-value methods, which optimize an action-value function. Policy gradient methods are enhanced by using an Actor-Critic architecture, as in algorithms such as A2C \cite{mnih_asynchronous_2016} and PPO \cite{schulman_proximal_2017}, which reduce variance in the policy gradient by using a learned value function (critic) to estimate the value of each state. Policy gradient methods have been used in many works on DRA in optical networks, such as A2C for DeepRMSA \cite{chen_deeprmsa_2019}. 
\end{itemize}

%Policy gradient methods are superior to action-value methods when the environment has stochastic dynamics (such as in a dynamic traffic scenario) due to their ability to learn stochastic policies \cite{sutton_reinforcement_2018}. It has been demonstrated that in many sequential decision-making problems, the policy is a simpler function to learn than an action-value function \cite{simsek_why_2016}. We therefore propose that policy gradient methods are better suited than action-value methods to DRA problems in optical networks.}

%\textbf{Model-based} RL algorithms use an explicit model of the environment's dynamics alongside the policy. The model may be an available simulator, as in AlphaGo \cite{silver_mastering_2016} or can be learned, as in MuZero \cite{silver_general_2018}. The model is used to simulate experience for a search process (e.g. Monte Carlo Tree Search) over possible sequences of actions, enabling multi-step planning to maximize reward. This leads to considerably higher performance in complex tasks, at the cost of much higher computational complexity \cite{brown_superhuman_2019}.

%Only model-free algorithms have been applied to DRA problems thus far in the research literature.


% \begin{equation}
%     \label{eq:bellman_optimality}
%     V^*(s) = \max_a \left( R(s,a) + \gamma \sum_{s'} P(s'|s,a) V^*(s') \right)
% \end{equation}
% Equation \ref{eq:bellman_optimality} is the Bellman optimality equation, a fundamental principle in RL that defines the optimal value function. It states that the optimal value of a state is equal to the expected return for the best action from that state. This equation forms the basis for many RL algorithms, including value iteration and Q-learning, and provides a mathematical framework for understanding how agents can make optimal decisions in sequential decision-making problems.

% \begin{equation}
%     \label{eq:bellman_optimality_q}
%     Q^*(s,a) = R(s,a) + \gamma \sum_{s'} P(s'|s,a) \max_{a'} Q^*(s',a')
% \end{equation}
% Equation \ref{eq:bellman_optimality_q}, the Q-function version of the Bellman optimality equation, defines the optimal action-value function in reinforcement learning. It represents the expected return of taking action a in state s and then following the optimal policy thereafter. This equation is crucial in Q-learning and other value-based methods, as it allows for optimal action selection without requiring a model of the environment. The Q-function directly incorporates the action into the value estimation, making it particularly useful for control problems.

==> 2_PAPER_SECTIONS/3_literature_survey.tex <==
\section{Literature Survey}
\label{sec:survey}

There exists a considerable body of literature on RL for DRA problems in optical networks. %\cite{amin_survey_2021}. 
DRA in optical networks is distinguished from similar problems in electronically linked networks by the nature of fiber optic links, which carry a set of wavelengths or FSU, defined by the ITU standards G.671 and G.694.2 \cite{international_telecommunication_union_spectral_2002,international_telecommunication_union_transmission_2012}. In this work we only consider publications related to optical networks but acknowledge the closely related literature on RL for other graph-based resource allocation problems.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{IMAGES/RL_RSA_litreview_barchart.png}
    \caption{Count of publications related to RL for resource allocation problems in optical networks. Citations for each classification category are: RWA \cite{garcia_multicast_2003,pointurier_reinforcement_2007,koyanagi_reinforcement_2009,suarez-varela_routing_2019,shiraki_dynamic_2019,shiraki_reinforcement-learning-based_2019,tzanakaki_self-learning_2020,zhao_cost-efficient_2021,freire-hermelo_dynamic_2021,liu_waveband_2021,nevin_techniques_2022,di_cicco_deep_2022,di_cicco_deepls_2023,nallaperuma_interpreting_2023}, RSA \cite{reyes_adaptive_2017,li_deepcoop_2020,li_multi-objective_2020,romero_reyes_towards_2021,zhao_reinforced_2021,wang_dynamic_2021,quang_magc-rsa_2022,cruzado_reinforcement-learning-based_2022,zhao_rsa_2022,jiao_reliability-oriented_2022,almasan_deep_2022,wu_service_2022,arce_reinforcement_2022,sharma_deep_2023,lin_deep-reinforcement-learning-based_2023,hernandez-chulde_experimental_2023,cheng_ptrnet-rsa_2024,chen_gsaddqn_2024}, RMSA \cite{chen_deeprmsa_2019,wang_resource_2020,shimoda_mask_2021,shi_deep-reinforced_2021,shimoda_deep_2021,sheikh_multi-band_2021,xu_spectrum_2021,chen_multi-task-learning-based_2021,gonzalez_improving_2022,bryant_q-learning_2022,terki_routing_2022,tang_deep_2022,cheng_routing_2022,xu_deep_2022,tang_heuristic_2022,tu_entropy-based_2022,momo_ziazet_deep_2022,pinto-rios_resource_2023,errea_deep_2023,beghelli_approaches_2023,terki_routing_2023,tanaka_pre-_2023,xu_hierarchical_2023,sadeghi_performance_2023,tang_routing_2023,teng_deep-reinforcement-learning-based_2024,xiong_graph_2024,teng_drl-assisted_2024,unzain_reinforcement_2024,zhou_opti-deeproute_2024,li_opticgai_2024,xie_physical_2024,yan_drl-based_2024}, Other \cite{boyan_packet_1993,ma_demonstration_2019,zhao_reinforcement-learning-based_2019,wang_subcarrier-slot_2019,luo_leveraging_2019,natalino_optical_2020,ma_co-allocation_2020,wang_deepcms_2020,weixer_reinforcement_2020,liu_multi-agent_2021,zhao_service_2021,tian_reconfiguring_2021,morales_multi-band_2021,tanaka_reinforcement-learning-based_2022,koch_reinforcement_2022,hernandez-chulde_evaluation_2022,etezadi_deepdefrag_2022,etezadi_deep_2023,tanaka_adaptive_2023,johari_drl-assisted_2023,zhang_admire_2023,fan_blocking-driven_2023,lian_dynamic_2024,li_tabdeep_2024,wang_availability-aware_2024,yin_dnn_2024,tse_reinforcement_2024,tanaka_reinforcement-learning-based_2024,doherty_xlron_2024,natalino_optical_2024,mccann_sdonsim_2024,jara_dream-gym_2024}.}
    \label{fig:lit_barchart}
\end{figure}



\subsection{Survey methodology}
\label{sec:survey-methodology}

%we searched the Google Scholar database using the following search terms: "'REINFORCEMENT LEARNING' AND 'NETWORK' AND ('OPTICAL' OR 'WAVELENGTH' OR 'SPECTRUM')". Papers were limited to English-language peer-reviewed articles. We filtered the search results by inspection of paper titles and abstracts, and manually added any related works from our own citation database that were missing from the initial search. A review of the collected papers then created the final set of 97.

To provide an overview of research progress on RL applied to DRA problems in optical networks, we searched to gather all relevant research papers. We performed a manual review of results from citation databases to create the final set of 97 peer-reviewed papers. Figure \ref{fig:lit_barchart} shows the count of papers by publication year. The papers are grouped in 4 categories: 'RWA', 'RSA', 'RMSA', and 'Other'. We use this set of papers for our analysis of benchmarking practices in the field, which we present in the next section with further commentary on Figure \ref{fig:lit_barchart}. 

%the 'Other' category of figure \ref{fig:lit_barchart}, which includes papers on RL applied to: traffic grooming \cite{tanaka_reinforcement-learning-based_2022,zhang_admire_2023,tanaka_adaptive_2023,tanaka_reinforcement-learning-based_2024}, defragmentation \cite{etezadi_deepdefrag_2022,fan_blocking-driven_2023,johari_drl-assisted_2023,etezadi_deep_2023}, survivability or service restoration \cite{zhao_reinforcement-learning-based_2019,luo_leveraging_2019,zhao_service_2021,hernandez-chulde_evaluation_2022,zhao_rsa_2022,luo_survivable_2022,jiao_reliability-oriented_2022}, multicast provisioning \cite{garcia_multicast_2003,tian_reconfiguring_2021,li_tabdeep_2024}, simulation training environments \cite{natalino_optical_2020,natalino_optical_2024,doherty_xlron_2024,mccann_sdonsim_2024}, and other problems such as transceiver parameter optimization \cite{weixer_reinforcement_2020,koch_reinforcement_2022,koch_high-generalizability_2022} or launch power optimization \cite{tse_reinforcement_2024}


\subsection{Review of benchmarking practices}
\label{sec:benchmarking_practices}


%To understand progress on RL applied to DRA problems in optical networks, it is essential to have standard benchmarks. Benchmarks refer to both the problem under investigation and the quality of the solution. In machine learning research, performance benchmarks on MNIST \cite{li_deng_mnist_2012} and ImageNet \cite{krizhevsky_imagenet_2012} have been vital to the astounding progress in that field. 


In optical networks research, the first benchmark for RL was established by DeepRMSA \cite{chen_deeprmsa_2019} (discussed in detail in Section \ref{sec:repro}). DeepRMSA was the first RL approach to achieve lower service blocking probability than KSP-FF, or any heuristic that considers multiple candidate paths. As a result of this breakthrough performance, and its open source codebase, the problem definition from DeepRMSA (topologies, traffic model, modulation format reach, FSU per link, etc.) became a de facto standard. Follow-up works used identical or similar problem definitions and compared to DeepRMSA on their problem \cite{xu_spectrum_2021,quang_magc-rsa_2022,errea_deep_2023,tang_heuristic_2022,xu_deep_2022,cheng_ptrnet-rsa_2024,yan_drl-based_2024,zhou_opti-deeproute_2024}. Arguably, comparing to DeepRMSA has become standard benchmarking practice.

%Although this comparison to the "state of the art" appears to be good practice, it is misguided. The performance of RL agents is highly sensitive to algorithmic details and hyperparameters \cite{engstrom_implementation_2020}, random seeds, and non-deterministic factors \cite{nagarajan_impact_2018}. Guidelines have been established for the reliable comparison of competing RL approaches \cite{henderson_deep_2019}. The comparisons to DeepRMSA in follow-up works have not followed these guidelines. For example, hyperparameters such as learning rate and discount factor should be tuned when applying an algorithm to a new setting. Consequently, the comparisons to DeepRMSA in follow-up works are not fair.

Previous work has called for more rigorous benchmarking practices for research on RL for optical networking \cite{di_cicco_deep_2022}, with recommendations for comparison against other machine learning approaches such as GA and PSO, in addition to estimated bounds on network blocking or throughput. Some studies of RL for resource allocation have restricted themselves to sufficiently small problem sizes and static traffic, to enable comparison to ILP results \cite{liu_waveband_2021,di_cicco_deep_2022,zhao_rsa_2022,momo_ziazet_deep_2022,di_cicco_deepls_2023}. Although this provides a reliable bound, it is not applicable to dynamic traffic.

Benchmarking against standard heuristic algorithms, such as KSP-FF, avoids the complexity of training a competing machine learning approach, performs deterministic allocation, and can scale to large problem instances. However, it is important to choose the best performing heuristic for a particular case of study as a benchmark. Of the papers that benchmark their RL solution to KSP-FF (or other heuristics that consider multiple candidate paths) \cite{chen_deeprmsa_2019,chen_multi-task-learning-based_2021,shi_deep-reinforced_2021,shimoda_deep_2021,xu_spectrum_2021,zhao_reinforced_2021,zhao_service_2021,shimoda_mask_2021,quang_magc-rsa_2022,tu_entropy-based_2022,tang_heuristic_2022,xu_deep_2022,cheng_routing_2022,nevin_techniques_2022,tang_deep_2022,di_cicco_deep_2022,terki_routing_2023,sadeghi_performance_2023,tanaka_adaptive_2023,tang_routing_2023,xu_hierarchical_2023,errea_deep_2023,hernandez-chulde_experimental_2023,cheng_ptrnet-rsa_2024,fan_blocking-driven_2023}, most achieve 20-30\% reduction in service blocking probability compared to their best heuristic. Only 3 papers achieve a reduction greater than this: MaskRSA \cite{shimoda_mask_2021}, PtrNet-RSA \cite{cheng_ptrnet-rsa_2024}, and Terki et al \cite{terki_routing_2022}. Despite these impressive results, we demonstrate in Section \ref{sec:repro_main} that MaskRSA and PtrNet-RSA are beaten by KSP-FF or FF-KSP by considering 50 candidate paths and ordering the paths by number of hops\footnotemark.

\footnotetext{We have not re-created the study of Terki et al. for benchmarking in Section \ref{sec:repro_main} as it is multi-band and out of scope of this work.
We hypothesise that their approach performs strongly because, similar to PtrNet-RSA, it is not limited to selecting from only K paths.}

Benchmarking is further complicated by the fast evolution of optical networking, with novel paradigms such as multi-band \cite{beghelli_approaches_2023} and multi-core \cite{pinto-rios_resource_2023} emerging, and the wide variety of network topologies \cite{matzner_topology_2024} and components that can be considered. The evolution of optical networks research is evidenced by growth in the 'Other' category of Figure \ref{fig:lit_barchart}, which includes papers on RL applied to: traffic grooming \cite{tanaka_reinforcement-learning-based_2022,zhang_admire_2023,tanaka_adaptive_2023,tanaka_reinforcement-learning-based_2024}, defragmentation \cite{etezadi_deepdefrag_2022,fan_blocking-driven_2023,johari_drl-assisted_2023,etezadi_deep_2023}, survivability or service restoration \cite{zhao_reinforcement-learning-based_2019,luo_leveraging_2019,zhao_service_2021,hernandez-chulde_evaluation_2022,zhao_rsa_2022,luo_survivable_2022,jiao_reliability-oriented_2022}, multicast provisioning \cite{garcia_multicast_2003,tian_reconfiguring_2021,li_tabdeep_2024}, %simulation training environments \cite{natalino_optical_2020,natalino_optical_2024,doherty_xlron_2024,mccann_sdonsim_2024}, 
and other problems such as transceiver parameter optimization \cite{weixer_reinforcement_2020,koch_reinforcement_2022,koch_high-generalizability_2022} or launch power optimization \cite{tse_reinforcement_2024}

The establishment of reliable benchmarks is made more difficult by the fragmented software environment for optical network simulations for RL. Several open source toolkits have been introduced to aid researchers and improve productivity, but none has proved sufficiently popular for it to become standard. Optical-rl-gym \cite{natalino_optical_2020} was the first paper to attempt to introduce a new standard library for this task. This was followed by an extension to multi-band environments \cite{morales_multi-band_2021} and in 2024 was further extended to include a more sophisticated physical layer model for lightpath SNR calculations, renamed as the Optical Networking Gym \cite{natalino_optical_2024}. Additionally, MaskRSA provides an open source simulation framework (RSA-RL) \cite{shimoda_mask_2021} and DeepRMSA's codebase is widely used \cite{chen_deeprmsa_nodate}. SDONSim \cite{mccann_sdonsim_2024} and DREAM-ON-GYM \cite{jara_dream-gym_2024} are other recent additions to the landscape of available simulation frameworks that further fragment the available options. 

In summary, progress in applying RL to DRA problems in optical networks has been difficult to quantify due to several factors. First, the lack of standardized benchmarking practices has made it challenging to fairly compare different approaches. Second, while some studies have used ILP solutions as benchmarks, these are limited to small problem sizes and static traffic scenarios, making them impractical for large-scale or dynamic applications. Third, multiple competing simulation frameworks %(Optical-rl-gym, RSA-RL, SDONSim, DREAM-ON-GYM) 
and publications without open source code have made it difficult to ensure consistent testing conditions across different studies. Finally, the rapid evolution of optical networking technology means benchmarks must constantly evolve to remain relevant. 

The lack of reliable benchmarks, and the resulting difficulty in assessing progress in the field, is what motivates our investigations of heuristic benchmarks in Section \ref{sec:heuristic_comparison} and their application to our recreation of previous work in Section \ref{sec:repro_main}.

%As we show in section \ref{sec:repro}, heuristic algorithms . This underscores the need for more rigorous and standardized evaluation methods in this field. 
% 

%In this work we use XLRON \cite{doherty_xlron_2023}, the framework introduced at Optical Fibre Communications (OFC) 2024 that we continue to develop. We outline its benefits and justify its use in Section \ref{sec:repro}.


\subsection{Recommendations for benchmarking best practice}
\label{sec:benchmarking_recommendations}

% Metnion that we do not allow extra cards 

Based on our review of the field, we make the following recommendations for selecting benchmarks and evaluating solutions to DRA problems in optical networks:

\begin{itemize}[itemsep=0pt]
    %\item Use standard problems where possible to facilitate comparison to previous work.
    \item \textbf{Benchmark selection}: Assess multiple benchmarks and select the best available. Tune parameters such as number of candidate paths and path sort criteria (see section 4\ref{sec:path_ordering}) to maximize performance. Prefer deterministic algorithms that can be reproduced without re-training ML components.
    \item \textbf{Statistical rigor}: Perform sufficient trials for statistical significance (minimum 100 blocking events is a rule of thumb) with multiple random seeds. Report mean and a measure of variability of results e.g. standard deviation.
    \item \textbf{Methodological transparency}: Be transparent in your choice of benchmark and its implementation details. Release code to facilitate verification and extension of research findings. Utilize established simulation frameworks where possible to minimize implementation discrepancies across studies, with unit tests to ensure correctness.
\end{itemize}

We implement these recommendations in our analyses in sections \ref{sec:heuristic_comparison} and \ref{sec:repro_main}. We note that these recommendations apply to the evaluation of any solution method for DRA problems, including RL, other ML approaches, or novel heuristic algorithms.






\subsection{Selection of papers for benchmarking}
\label{sec:paper_summaries}

To assess progress in RL for DRA, we select 5 papers to re-benchmark in section \ref{sec:repro_main}. We select these papers primarily because they all compare their results to "DeepRMSA"\footnotemark with similar traffic models and topologies, therefore present the most consistent application of benchmarks in the field. We also select based on their impact, which we assess by qualitative and quantitative criteria. The qualitative criteria are novelty, contribution, and reputation of publication or conference. The quantitative criterion is their blocking performance relative to benchmarks. They are also among the most highly cited papers in the field, as of April 2025.

\footnotetext{We note that the training of RL solutions is highly sensitive to hyperparameters \cite{engstrom_implementation_2020} and non-deterministic factors \cite{nagarajan_impact_2018}, therefore the comparisons that the selected papers make to re-trained DeepRMSA agents may not be robust.}


\begin{enumerate}[itemsep=0pt]
    \item \textbf{DeepRMSA} \cite{chen_deeprmsa_2019} constructs a feature matrix to represent the available paths for the current requests and applies a NN with 5 x 128 hidden units to select from the K-shortest paths with first-fit spectrum allocation. It demonstrates service blocking probability (SBP) reduced by 20\% vs. KSP-FF on the NSFNET and COST239 topologies. DeepRMSA's impact was enhanced by its open source codebase. %published 2019, has over 178 citations.
    \item \textbf{Reward-RMSA} \cite{tang_heuristic_2022} builds on the DeepRMSA framework and changes the reward function to incorporate fragmentation-related information. They report SBP reduced by 32\% vs. multiple heuristics and 55\% vs. DeepRMSA on NSFNET and COST239. %published 2022, has over 22 citations.
    \item \textbf{GCN-RMSA} \cite{xu_deep_2022} is notable as the first work to use advanced NN architectures to improve performance. They use a graph convolutional network (GCN) (including recurrent neural network (RNN) as the path aggregation function) in the policy and value functions, which they claim allows improved feature extraction from the network state. Like DeepRMSA and Reward-RMSA, the policy selects from K paths with first-fit spectrum allocation. They report SBP reduced by up to 30\% vs. multiple heuristics and 18\% vs. DeepRMSA. on NSFNET, COST239, and USNET. %published 2022, has over 36 citations
    \item \textbf{MaskRSA} \cite{shimoda_mask_2021} innovated by selecting from the entire range of available slots on the K paths and using invalid action masking \cite{huang_closer_2022} to increase the efficiency of training. Despite the RSA in the title, the paper does consider distance-dependent modulation format (RMSA). MaskRSA presented improvements over KSP-FF on NSFNET and JPN48 topologies with over an order of magnitude lower SBP, or a 35-45\% increase in the supported traffic in their cases of study. The authors of MaskRSA also contributed to open source by releasing their simulation framework, RSA-RL. %published 2021, has over 28 citations
    \item \textbf{PtrNet-RSA} \cite{cheng_ptrnet-rsa_2024}, newly published in 2024. It innovates in both the problem setting and its use of pointer-nets \cite{vinyals_pointer_2015}. The pointer-net is used to select the constituent nodes of the target path, thereby removing the restriction of selecting from the pre-calculated K-shortest paths. Invalid action masking is used to allow selection from all available spectral slots. Additionally, the paper considers joint optimization of the mean path SNR and the SBP through its reward function. It demonstrates SBP reduced by over an order of magnitude vs. KSP-FF and their implementation of MaskRSA on NSFNET, COST239, and USNET.
\end{enumerate}


%Although this comparison to the "state of the art" appears to be good practice, it is misguided. The performance of RL agents is highly sensitive to algorithmic details and hyperparameters \cite{engstrom_implementation_2020}, random seeds, and non-deterministic factors \cite{nagarajan_impact_2018}. Guidelines have been established for the reliable comparison of competing RL approaches \cite{henderson_deep_2019}. The comparisons to DeepRMSA in follow-up works have not followed these guidelines. For example, hyperparameters such as learning rate and discount factor should be tuned when applying an algorithm to a new setting. Consequently, the comparisons to DeepRMSA in follow-up works are not fair.





% \subsection{Research trends}
% \label{sec:trends}

% Our analysis of the literature reveals several significant trends:

% \textbf{Timeline and Technology Adoption: }
% A marked increase in publications began in 2019, following the influential DeepRMSA paper \cite{chen_deeprmsa_2019}. This represents a 5-6 year lag between breakthrough ML publications (e.g. Deep RL for Atari in 2013 \cite{mnih_human-level_2015}) and adoption in optical networking. Publication activity peaked in 2022, with a notable dip in 2020 due to the COVID-19 pandemic.

% \textbf{Evolution of Problem Focus: }
% Early work (pre-2019) predominantly addressed RWA but RWA publications have declined since, with no publications in 2024. Research attention has shifted toward RMSA. Recent work also increasingly addresses specialized problems beyond basic routing and spectrum allocation, as seen by the rise in "Other" categories.

% \textbf{Research Maturity and Diversification: }
% The growth in "Other" categories suggests researchers are seeking new directions. Recent publications show movement toward novel application areas with potentially greater performance gains, such as multi-objective optimization \cite{nallaperuma_interpreting_2023}, joint optimization of blocking and lightpath signal-to-noise ratio (SNR) \cite{cheng_ptrnet-rsa_2024,xie_physical_2024,teng_deep-reinforcement-learning-based_2024,yan_drl-based_2024} or channel launch power \cite{xiao_channel_2024}. We hypothesise this shift may be partly motivated by a saturation of performance improvements in simpler RWA/RSA/RMSA problems, which we investigate in section \ref{sec:bounds}.



% \subsection{Recommendations for reporting metrics and reproducibility}
% \label{sec:recommendations}
% Based on the above review, we make  recommendations to improve the quality and reproducibility of results:

% \textbf{Improved metrics}

% For a more meaningful performance comparisons, several metrics could be refined, as outlined in this section.

% - Network data throughput: use bitrate blocking probability (BBP) rather than service blocking probability (SBP) to quantify network blocking.  Key when traffic requests have diverse bitrate requirements. For RWA or uniform bitrate traffic, BBP and SBP are equivalent. 

% Consider the approach of Shiraki et al. \cite{shiraki_dynamic_2019} and Cruzado et al. \cite{cruzado_capacity-bound_2024} of setting a target blocking probability (e.g., 0.1\%) and comparing solutions based on the maximum traffic load that can be supported. Data traffic in Tbps is a more easily interpreted and physically meaningful measure than blocking probability.This is used to present network blocking bounds in Section \ref{sec:bounds}. We believe that researchers have preferred to report on blocking probability as it allows headline results to appear more impressive (e.g. "one order of magnitude reduction") than the equivalent relative change in supported traffic



% \textbf{Statistical Significance:}
% Many works do not include sufficient trials to establish statistical significance, particularly when blocking events are rare. It is proposed that the following steps are followed:
% \begin{itemize}[itemsep=0pt]
%     \item Obtain a sufficient number of blocking events (minimum 100) to have >95\% confidence in mean blocking estimate
%     \item Ensure different random seeds are used for parallel training or evaluation runs
%     \item Publish uncertainty estimates along with mean performance metrics
%     \item Use multiple random seeds (minimum 5) for both training and evaluation
% \end{itemize}

% \textbf{Reproducibility:}
% We propose to compare network blocking from deterministic heuristic algorithms. When comparing against existing RL solutions, we emphasise the following:
% \begin{itemize}[itemsep=0pt]
%     \item Hyperparameters must be re-tuned when the problem setting differs from the original paper
%     \item Equivalent computing resources should be devoted to performing hyperparameter sweeps for and training competing solutions
%     \item All code should be made publicly available, with instructions to reproduce published results.

    
% \end{itemize}





















%%%%%%%%%%%%%%%%%%

%Shi et al. showed progress in the problem setting by including a simple lightpath SNR calculation to the network physical layer model, and calculating the highest available modulation format on the basis of SNR instead of maximum reach \cite{shi_deep-reinforced_2021}. They make this minor addition and otherwise use the same algorithmic setup as DeepRMSA.

%Unusually, a negative result was accepted for publication at ONDM 2021 on RL for multi-band RMSA \cite{sheikh_multi-band_2021}. This can partially be explained by interest in the relatively novel problem setting but perhaps also indicates that progress on the application of RL to this problem and similar was stalling.


% Could complete the argument by saying that the solutions provided by the defragmentation method are entirely physically realistic, therefore present a hard upper bound on network capacity, in comparison to the cut-sets method which may be tighter than necessary due to sub-optimal spectrum allocation.
%% IDEA: the best upper bound would probably be to do cut-sets with defragmented spectrum i.e. just do cut-sets with scalar capacity on each link, i.e. just do the traditional max-flow min-cut theorem but with the defragmented spectrum. This would be the most physically realistic upper bound. Could be a good future work idea.


% Specifically, the successor works that use the DeepRMSA codebase are . Note that 

% The direct successor works are from Chen et al using the DeepRMSA framework with transfer learning on different topologies and traffic \cite{chen_multi-task-learning-based_2021}, Tang et al using a shaped reward function to improve performance, Xu et al using graph and recurrent neural networks to for the policy network to improve performance \cite{xu_deep_2022}, Xu et al investigate a hierarchical framework for multi-domain networks \cite{xu_hierarchical_2023}, Errea et al use DeepRMSA with two choices of first slots per path \cite{errea_deep_2023}, a modification that was investigated in the original DeepRMSA paper. DeepRMSA has also been used as a benchmark in MaskRSA \cite{shimoda_mask_2021} and PtrNet-RSA \cite{cheng_ptrnet-rsa_2024}.

















%%%%%%%%%%%%%%%%%%





% 0  DeepRMSA: A Deep Reinforcement Learning Framew...     chen_deeprmsa_2019
% 1  Mask RSA: End-To-End Reinforcement Learning-ba...      shimoda_mask_2021
% 2  Techniques for applying reinforcement learning...  nevin_techniques_2022
% 3  The Optical RL-Gym: An open-source toolkit for...  natalino_optical_2020
% 4  Heuristic Reward Design for Deep Reinforcement...    tang_heuristic_2022

% Total entries: 97
% Matched entries: 97
% Matching rate: 100.00%
% Papers classified as 'Other':
% - The Optical RL-Gym: An open-source toolkit for applying reinforcement learning in optical networks
% - Reconfiguring multicast sessions in elastic optical networks adaptively with graph-aware deep reinforcement learning
% - DRL-Assisted Reoptimization of Network Slice Embedding on EON-Enabled Transport Networks
% - Blocking-Driven Spectrum Defragmentation Based on Deep Reinforcement Learning in Tidal Elastic Optical Networks
% - DeepDefrag: A deep reinforcement learning framework for spectrum defragmentation
% - Multi-band Environments for Optical Reinforcement Learning Gym for Resource Allocation in Elastic Optical Networks
% - TABDeep: A two-level action branch architecture-based deep reinforcement learning for distributed sub-tree scheduling of online multicast sessions in EON
% - Reinforcement-learning-based path planning in multilayer elastic optical networks [Invited]
% - Adaptive Traffic Grooming Using Reinforcement Learning in Multilayer Elastic Optical Networks
% - Reinforcement-Learning-based Multilayer Path Planning Framework that Designs Grooming, Route, Spectrum, and Operational Mode
% - ADMIRE: collaborative data-driven and model-driven intelligent routing engine for traffic grooming in multi-layer X-Haul networks
% - Packet Routing in Dynamically Changing Networks: A Reinforcement Learning Approach
% - Reinforcement Learning for Power Management in Low-margin Optical Networks
% - DNN distributed inference offloading scheme based on transfer reinforcement learning in metro optical networks
% - Availability-Aware and Delay-Sensitive RAN Slicing Mapping Based on Deep Reinforcement Learning in Elastic Optical Networks
% - DREAM-ON GYM: A Deep Reinforcement Learning Environment for Next-Gen Optical Networks:
% - Dynamic slicing of multidimensional resources in DCI-EON with penalty-aware deep reinforcement learning
% - DeepCMS <sup>3</sup> : A Deep Reinforcement Learning Framework for Core, Mode and Spectrum Sequential Scheduling over Optical Transport Network
% - A Subcarrier-Slot Autonomous Partition Scheme Based on Deep-Reinforcement-Learning in Elastic Optical Networks
% - Reinforcement-Learning-Based Multi-Failure Restoration in Optical Transport Networks
% - Demonstration of Image Processing Based on Reinforcement Learning in Multi-Modal Optical Transport Networks
% - Co-Allocation of Service Routing in SDN-driven 5G IP+Optical Smart Grid Communication Networks based on Deep Reinforcement Learning
% - Service restoration in multi-modal optical transport networks with reinforcement learning
% - Multi-Agent Federated Reinforcement Learning for Privacy-enhanced Service Provision in Multi-domain Optical Network
% - Evaluation of Deep Reinforcement Learning for Restoration in Optical Networks
% - Deep reinforcement learning for proactive spectrum defragmentation in elastic optical networks
% - XLRON: Accelerated Reinforcement Learning Environments for Optical Networks
% - Reinforcement Learning for Generalized Parameter Optimization in Elastic Optical Networks
% - Optical Networking Gym: an open-source toolkit for resource assignment problems in optical networks
% - SDONSim: An Advanced Simulation Tool for Software-Defined Elastic Optical Networks
% - Leveraging double-agent-based deep reinforcement learning to global optimization of elastic optical networks with enhanced survivability
% - A Reinforcement Learning Framework for Parameter Optimization in Elastic Optical Networks

% Papers classified as 'Routing':

% Tag distribution:
% RMSA: 33 (34.02%)
% Other: 32 (32.99%)
% RSA: 18 (18.56%)
% RWA: 14 (14.43%)

% Total papers: 97

% First few rows of the updated DataFrame:
%                                                Title  \
% 0  DeepRMSA: A Deep Reinforcement Learning Framew...   
% 1  Mask RSA: End-To-End Reinforcement Learning-ba...   
% 2  Techniques for applying reinforcement learning...   
% 3  The Optical RL-Gym: An open-source toolkit for...   
% 4  Heuristic Reward Design for Deep Reinforcement...   

%                 Manual Tags Priority_Tag  
% 0                  RL; RMSA         RMSA  
% 1  RL; RMSA; Action masking         RMSA  
% 2      RL; RWA; Incremental          RWA  
% 3        RL; Other; Toolkit        Other  
% 4                  RL; RMSA         RMSA  
% Citation tags for each priority tag class, sorted by publication date:

% Other:
% boyan_packet_1993,ma_demonstration_2019,zhao_reinforcement-learning-based_2019,wang_subcarrier-slot_2019,luo_leveraging_2019,natalino_optical_2020,ma_co-allocation_2020,wang_deepcms_2020,weixer_reinforcement_2020,liu_multi-agent_2021,zhao_service_2021,tian_reconfiguring_2021,morales_multi-band_2021,tanaka_reinforcement-learning-based_2022,koch_reinforcement_2022,hernandez-chulde_evaluation_2022,etezadi_deepdefrag_2022,etezadi_deep_2023,tanaka_adaptive_2023,johari_drl-assisted_2023,zhang_admire_2023,fan_blocking-driven_2023,lian_dynamic_2024,li_tabdeep_2024,wang_availability-aware_2024,yin_dnn_2024,tse_reinforcement_2024,tanaka_reinforcement-learning-based_2024,doherty_xlron_2024,natalino_optical_2024,mccann_sdonsim_2024,jara_dream-gym_2024

% RMSA:
% chen_deeprmsa_2019,wang_resource_2020,shimoda_mask_2021,shi_deep-reinforced_2021,shimoda_deep_2021,sheikh_multi-band_2021,xu_spectrum_2021,chen_multi-task-learning-based_2021,gonzalez_improving_2022,bryant_q-learning_2022,terki_routing_2022,tang_deep_2022,cheng_routing_2022,xu_deep_2022,tang_heuristic_2022,tu_entropy-based_2022,momo_ziazet_deep_2022,pinto-rios_resource_2023,errea_deep_2023,beghelli_approaches_2023,terki_routing_2023,tanaka_pre-_2023,xu_hierarchical_2023,sadeghi_performance_2023,tang_routing_2023,teng_deep-reinforcement-learning-based_2024,xiong_graph_2024,teng_drl-assisted_2024,unzain_reinforcement_2024,zhou_opti-deeproute_2024,li_opticgai_2024,xie_physical_2024,yan_drl-based_2024

% RSA:
% reyes_adaptive_2017,li_deepcoop_2020,li_multi-objective_2020,romero_reyes_towards_2021,zhao_reinforced_2021,wang_dynamic_2021,quang_magc-rsa_2022,cruzado_reinforcement-learning-based_2022,zhao_rsa_2022,jiao_reliability-oriented_2022,almasan_deep_2022,wu_service_2022,arce_reinforcement_2022,sharma_deep_2023,lin_deep-reinforcement-learning-based_2023,hernandez-chulde_experimental_2023,cheng_ptrnet-rsa_2024,chen_gsaddqn_2024

% RWA:
% garcia_multicast_2003,pointurier_reinforcement_2007,koyanagi_reinforcement_2009,suarez-varela_routing_2019,shiraki_dynamic_2019,shiraki_reinforcement-learning-based_2019,tzanakaki_self-learning_2020,zhao_cost-efficient_2021,freire-hermelo_dynamic_2021,liu_waveband_2021,nevin_techniques_2022,di_cicco_deep_2022,di_cicco_deepls_2023,nallaperuma_interpreting_2023

% Date range for each tag class:
% RMSA: 2019 - 2024
% RWA: 2003 - 2023
% Other: 1993 - 2024
% RSA: 2017 - 2024







% K-paths used but not beaten: \cite{sheikh_multi-band_2021,zhao_cost-efficient_2021}
% K-paths beaten: \cite{chen_deeprmsa_2019,chen_multi-task-learning-based_2021,,shi_deep-reinforced_2021,shimoda_deep_2021,xu_spectrum_2021,zhao_reinforced_2021,zhao_service_2021,shimoda_mask_2021,quang_magc-rsa_2022,terki_routing_2023,tu_entropy-based_2022,tang_heuristic_2022,xu_deep_2022,cheng_routing_2022,nevin_techniques_2022,tang_deep_2022,di_cicco_deep_2022,fan_blocking-driven_2023,sadeghi_performance_2023,tanaka_adaptive_2023,tang_routing_2023,xu_hierarchical_2023,errea_deep_2023,hernandez-chulde_experimental_2023,cheng_ptrnet-rsa_2024}
% ILP: \cite{liu_waveband_2021,di_cicco_deep_2022,zhao_rsa_2022,momo_ziazet_deep_2022,di_cicco_deepls_2023}
% DeepRMSA as benchmark: \cite{xu_spectrum_2021,quang_magc-rsa_2022,errea_deep_2023,tang_heuristic_2022,xu_deep_2022,cheng_ptrnet-rsa_2024,yan_drl-based_2024,zhou_opti-deeproute_2024}


% - DeepRMSA became a benchmark
% - I want to make the point that it is difficult to establish long-lived standard problems in optical networks as the field evolves quickly and new operating paradigms (such as multi-band andm utli-core) are consistently emerging.
% - 

% \cite{henderson_deep_2019} Deep Reinforcement Learning That Matters - general good practice (i.e.e epxeirmental reporting and procedure) for reproducibility of RL results
% \cite{nagarajan_impact_2018}  Impact of non-determinism in RL
% \cite{engstrom_implementation_2020} Sensitivity of PPO to code-level optimizations and implementation details




==> 2_PAPER_SECTIONS/4_heuristic_comparison.tex <==
\section{Heuristic algorithm benchmark evaluation}
\label{sec:heuristic_comparison}

To evaluate the results of the selected papers from Section \ref{sec:survey}\ref{sec:paper_summaries}, we must determine the best (lowest blocking probability) heuristic algorithms to use as benchmarks. In this section, we present comparisons of the heuristics listed in Table \ref{tab:heuristics}, evaluated on different traffic loads, topologies, and considering different numbers of candidate paths (K). On the basis of this analysis, we select the benchmarks to apply in section \ref{sec:repro_main}. We also include a discussion of the effect of different sort criteria for candidate paths in Section \ref{sec:path_ordering}, which significantly affects the blocking performance.

We select the algorithms in Table \ref{tab:heuristics} because they are commonly used as benchmarks or have been reported as superior to other heuristics.


\begin{table}[h]
\begin{tabular}{l|l|l}
Heuristic                         & Acronym & Reference                \\ \hline
K-Shortest Paths First-Fit        & KSP-FF  & \cite{zang_review_2000} \\
First-Fit K-Shortest Paths        & FF-KSP  & \cite{vincent_scalable_2019} \\
K-Shortest Paths Best-Fit         & KSP-BF  & \cite{abkenar_best_2016} \\
Best-Fit K-Shortest Paths         & BF-KSP  & \cite{abkenar_best_2016} \\
K-Minimum Entropy First-Fit       & KME-FF  & \cite{wright_minimum-_2015} \\
%K-Minimum Cut First-Fit           & KMC-FF  & \cite{tang_heuristic_2022} \\
%K-Minimum Frag First-Fit & KMF-FF  & \cite{tang_heuristic_2022} \\
K-Congestion Aware First-Fit      & KCA-FF  & CA2 from \cite{savory_congestion_2014}
\end{tabular}
\caption{RMSA heuristics used for benchmarking.}
\label{tab:heuristics}
\end{table}

%We also evaluated the K-Minimum Cut First-Fit (KMC-FF) and K-Minimum Frag First-Fit (KMF-FF) heuristics from Reward-RMSA \cite{tang_heuristic_2022}. These heuristics produce higher blocking probability than others when paths are ordered by number of hops. We exclude these results to improve the clarity of Figures \ref{fig:heur_comp}, \ref{fig:k_traffic}, and \ref{fig:heur_traffic}.

\begin{figure}
  \includegraphics[width=1.01\linewidth]{IMAGES/networks_plots_short.png}
  \caption{Network topologies used in our case studies from: DeepRMSA, Reward-RMSA, GCN-RMSA, MaskRSA, PtrNet-RSA \cite{chen_deeprmsa_2019} \cite{tang_heuristic_2022} \cite{xu_deep_2022} \cite{shimoda_mask_2021} \cite{cheng_ptrnet-rsa_2024}. We note that the USNET topology differs between GCN-RMSA and PtrNet-RSA. We show the GCN-RMSA version here. PtrNet-RSA also uses a variant of the COST239 topology.} %The COST239 topology shown is from DeepRMSA, the USNET is from PtrNet-RSA.}
  \label{fig:network_plots}
\end{figure}

Figure \ref{fig:network_plots} shows the topologies used in the selected papers. The node and link count for each topology is: NSFNET (14, 22), COST239 (11, 25), USNET (24, 43), JPN48 (48, 82). We use these topologies to analyze the performance of the heuristic algorithms and in our recreation of the papers' problems in section \ref{sec:repro_main}. %Some characteristic features of the topologies are summarised in table \ref{tab:topology_features}. 
We make all topology data available in our open source codebase \cite{michael_doherty_2024_jocn_xlron_2024}.



\subsection{Effect of path ordering}
\label{sec:path_ordering}

All the heuristics in Table \ref{tab:heuristics} select from the available pre-computed paths on the basis of sort criteria. The primary criterion may be a measure of the path congestion (KCA-FF), spectral fragmentation (KME-FF), or length (KSP-FF). In the event of multiple paths with equal value, a default ordering (usually ascending order of length) determines the selected path.

Conventionally, path length is considered as distance in km. However, we find that considering path length as number of hops (with length in km as a secondary sort criterion), significantly improves the performance of the heuristics. This has been observed previously by Baroni \cite{baroni_routing_1998}, who referred to it as Minimum Number of Hops routing (MNH). The intuitive explanation for this is that, if two paths can support the same order of modulation format, the path that comprises fewer links occupies fewer spectral resources. 

We refer to these two orderings as path length in km (\#km) or path length in number of hops (\#hops). Our comparisons of KSP-FF for these two orderings in Section \ref{sec:repro_main} Figure \ref{fig:repro} evidence the reduction in blocking probability from \#hops ordering. In our comparisons of heuristics in the next section, we use \#hops ordering.



\subsection{Simulation setup}

For each heuristic and topology, we carried out three simulation scenarios to investigate the effects of varying traffic loads and values of K on the relative blocking performance of the heuristics. 

\vspace{0.1cm}

\noindent \textbf{Experiment 1} - Increasing K:
\par \noindent \textbf{Aim}: Investigate relative performance of heuristics with increasing K. \textbf{Method}: Record service blocking probability (SBP) for each heuristic at values of K ranging from 2 to 26 at fixed traffic load. We arbitrarily select the traffic load for each topology so that the heuristics give a SBP of  $\sim$1\%.

\vspace{0.1cm}

\noindent \textbf{Experiment 2} - Increasing K at high to low traffic: 
\par \noindent \textbf{Aim}: Investigate the effect of increasing K at different traffic loads. \textbf{Method}: Record SBP at K ranging from 2 to 40 for a range of traffic loads. We select the traffic loads for each topology such that they result in 10$^{-5}$ to 10$^{-1}$ SBP. To simplify the analysis and plots, we only present results for KSP-FF.

\vspace{0.1cm}

\noindent \textbf{Experiment 3} - Increasing traffic load at K=50: 
\par \noindent \textbf{Aim}: Using the findings from Experiments 1 and 2, determine the lowest-blocking heuristic with optimized K-value across traffic loads. \textbf{Method}: Record SBP for high K (K=50) at varying traffic loads. We select the traffic loads for each topology such that they result in a range of SBP (10$^{-5}$ to 10$^{-1}$). This experiment provides evidence on which heuristic is the best overall for each topology.

\vspace{0.1cm}

For each experiment and heuristic, data was collected from 3000 independent trials with unique random seeds. The SBP was calculated after 10,000 connection requests, with the mean and standard deviation calculated across trials. Each data point in Figure \ref{fig:heuristic_combined} therefore shows summary statistics from 30 million connection requests, which gives high confidence in our results.

We considered dynamic traffic with fixed mean service holding time at 10 units. We considered the same traffic model and other settings as DeepRMSA\footnotemark: uniform traffic probability between each node pair, Poissonian arrival and departure statistics, uniform random selection of data rate from 25 to 100Gbps in 1Gbps intervals, and distance-dependent modulation formats from BPSK, QPSK, 8QAM, 16QAM, and maximum transmission distances of 10,000km, 2500km, 1250km, 625km, respectively,  We consider topologies with dual fibre links (one for each direction of propagation), 12.5GHz FSU width, and 100 FSU per fibre.

\footnotetext{We consider the DeepRMSA problem settings in these experiments because it is used by most of the papers presented in Section \ref{sec:repro_main}.} %For the same reason, we report our results in terms of SBP, despite our recommendation to use BBP in Section \ref{sec:recommendations}.}

\subsection{Results and discussion}

\textbf{Experiment 1} results in Figure \ref{fig:heuristic_combined}(a) show different outcomes for smaller networks (NSFNET and COST239) and larger networks (USNET and JPN48). For NSFNET and COST239, KSP-FF and KME-FF are approximately equal and give the lowest blocking. Their blocking decreases to a minimum for approximately K=23 and above for NSFNET and continues to decrease for K>26 for COST239.

For USNET and JPN48, FF-KSP is clearly the best heuristic, with blocking reduced by half for JPN48. Blocking from FF-KSP decreases with K until K=26 for USNET and continues dropping sharply for K>26 for JPN48. For USNET, KSP-FF and KME-FF become competitive with FF-KSP at large K. It can be argued that FF-KSP performs better in networks with higher numbers of nodes and links where there are many viable paths between source and destination, and dense packing of utilized wavelengths increases in relative importance to path selection.

The results from Experiment 1 indicate that KSP-FF and FF-KSP generally give the lowest blocking, depending on the network topology, and blocking decreases monotonically with increasing K. This experiment looked at a moderately high traffic load ($\sim$1\% SBP), therefore experiment 2 investigates if the effect of increasing K holds at different traffic loads. 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{IMAGES/heuristic_combined.png}
    \caption{Comparison of heuristic algorithms. (a) Service blocking probability (SBP) at fixed traffic and varying numbers of candidate paths (K). (b) SBP for KSP-FF at varying traffic loads and K=2 to K=40. (c) SBP at varying traffic load for K=50. The mean and standard deviation (shaded area) are calculated from 3000 trials of 10,000 traffic requests per data point. KSP-FF or FF-KSP with K=50 are found to give the lowest blocking.}
    \label{fig:heuristic_combined}
\end{figure*}



% \begin{figure*}[p]
%   \includegraphics[width=\textwidth]{IMAGES/heuristic_comparison.png}
%   \caption{Service blocking probability (SBP) for heuristics at fixed traffic and varying numbers of candidate paths (K). The mean and standard deviation (shaded area) are calculated from 3000 trials of 10,000 traffic requests per data point. Increasing K decreases the SBP for most heuristics. KSP-FF and FF-KSP give lowest SBP, depending on topology.}
%   \label{fig:heur_comp}

%   \vspace{1em}
%   \includegraphics[width=0.97\textwidth]{IMAGES/k_traffic_comparison.png}
%   \caption{Service blocking probability (SBP) for KSP-FF at varying traffic loads and K values. The mean and standard deviation (shaded area) are calculated from 3000 trials of 10,000 traffic requests per data point. For all traffic loads, increasing K decreases SBP for KSP-FF. Improvements saturate at high K.}
%   \label{fig:k_traffic}

%   \vspace{1em}
%   \includegraphics[width=\textwidth]{IMAGES/heuristic_50_traffic_comparison.png}
%   \caption{Service blocking probability (SBP) for heuristics at varying traffic load for K=50. The mean and standard deviation (shaded area) are calculated from 3000 trials of 10,000 traffic requests per data point. KSP-FF is the best heuristic for NSFNET and COST239. FF-KSP is best for USNET and JPN48.}
%   \label{fig:heur_traffic}
% \end{figure*}


\textbf{Experiment 2} results in Figure \ref{fig:heuristic_combined}(b) show that, regardless of the traffic load, increasing K decreases the SBP, until SBP reaches a minimum and increasing K does not decrease SBP further. Across all topologies and traffic loads tested in our experiments, we found that SBP does not decrease significantly for K>50. For very high traffic (approximately equivalent to incremental loading), the value of K beyond which SBP does not continue to decrease can be much lower.

\textbf{Experiment 3} results in Figure \ref{fig:heuristic_combined}(c) show the variation of SBP with traffic load for each heuristic with K=50. We verified that at least 50 unique paths are possible for every node pair on our investigated topologies. We select K=50 on the basis of experiments 1 and 2. These results confirm the initial findings from Experiment 1 - that KSP-FF and KME-FF are the lowest blocking for NSFNET and COST239\footnotemark, while FF-KSP is better for USNET and JPN48, with an order of magnitude lower blocking probability on JPN48 compared to the next best heuristic.

\footnotetext{Although Figure \ref{fig:heuristic_combined}(c) shows KME-FF gives slightly lower blocking than KSP-FF at lower traffic, we prefer KSP-FF for benchmarking purposes because of its widespread use and its greater simplicity.}

% \begin{figure*}
%   \includegraphics[width=\textwidth]{IMAGES/heuristic_50_traffic_comparison.png}
%   \caption{Comparison of service blocking probability from heuristic algorithms at varying traffic load for K=50.}
%   \label{fig:heur_traffic}
% \end{figure*}


In summary, we highlight the generally strong performance of the KSP-FF and FF-KSP heuristics but do not draw conclusions as to which is best in general, and encourage thorough analysis to determine the strongest heuristic benchmark for a particular problem, as we have exemplified here. Our analysis of heuristic algorithms is not exhaustive, and there may exist more advanced heuristics that are superior. We also emphasize the importance of selecting optimal path ordering for heuristics, as this can have a significant impact on performance. We find \#hops ordering is superior to \#km for reduced blocking probability, as evidenced in Section \ref{sec:repro_main} Figure \ref{fig:repro}.



==> 2_PAPER_SECTIONS/5_reproduction_of_published_results.tex <==
\section{Benchmarking of previous work}
\label{sec:repro_main}

As discussed in our literature review (Section \ref{sec:survey}), it is difficult to assess progress in the field due to several factors, particularly the diversity of problem definitions and use of weak benchmarks. To address this, we exactly recreate the problem settings from five influential papers from the literature, and apply the best-performing heuristics from Section \ref{sec:heuristic_comparison} in each case.

In this section, we first provide analysis of holding time truncation, an implementation detail present in the DeepRMSA codebase that significantly affects the blocking probability. We then present the results of our reproductions of the selected papers and compare to the heuristics, which have significantly lower blocking probability all of the published RL solutions.

We have corresponded with the authors of the selected papers to clarify details of their implementation and ensure that our recreations exactly match all the relevant details of their problems. We point out that we do not reproduce the training of the published RL results. We choose not to reproduce training because of insufficient training details and the widely documented difficulties in reproduction of RL training due to sensitivity to hyperparameters and random seeds \cite{henderson_deep_2019,engstrom_implementation_2020}. Extracting RL results from published papers results in a more reliable and fair comparison.

%DeepRMSA, Reward-RMSA, and GCN-RMSA use the same original DeepRMSA codebase as the basis for their experiments. Consequently, they all feature service holding time truncation, discussed in section \ref{sec:holding_time}. Another common characteristic is they use directed graphs with dual fiber links i.e. each link comprises two fibers, one for each direction of propagation. This doubles the maximum potential capacity of the network compared to single-fiber links. MaskRSA and PtrNet-RSA model single-fiber links, which makes the problem less challenging for RL due to less sparse reward signals \cite{nevin_techniques_2022} (more frequent blocking). PtrNet-RSA considers fixed bandwidth requests (no distance-dependent modulation format).

 We use our high-performance simulation framework, \mbox{XLRON} \cite{doherty_xlron_2023}, for all experiments. It has demonstrated 10x faster execution on CPU and over 1000x faster when parallelized on GPU compared to optical-rl-gym \cite{doherty_xlron_2024}. This is possible due to its array-based data model and use of the JAX numerical array computing framework, that enables just-in-time compilation to accelerator hardware. It also offers a complete suite of unit tests for core functionality, making it reliable, and includes features to reproduce the problem settings of the selected papers. We use it for these reasons and for its simple command-line interface, which facilitates experiment automation and reproducibility.













% \subsection{Simulation warm-up}
% \label{sec:warmup}

% To exactly recreate the problems from the selected papers, we generate the same number of traffic requests as the original study. This includes the connection requests that are generated to pre-populate the network until the blocking probability reaches steady-state, a phenomenon which is well-known in discrete-event simulation \cite{banks_discrete-event_2005}. We call the period prior to steady-state the warm-up period. 

% Warm-up is important so that the blocking probability reaches its steady-state value and is not an underestimate. This is known as the simulation start-up problem or the initial transient \cite{white_problem_2009}. %When training an RL agent, warm-up may help prevent primacy bias \cite{nikishin_primacy_2022}, where models overfit to data seen early in training. Starting with an empty network, initial traffic requests are trivially allocated due to abundant resources, providing no useful optimization signal. Training on a congested network with both successful and failed allocations gives more meaningful training data from the start.

% While most papers do not explicitly discuss warm-up, all of the selected papers use it. We therefore analyze the minimum required warm-up period for different traffic levels.

% \subsubsection{Experiment setup}

% We simulate a non-blocking network to determine the maximum\footnotemark number of requests needed to reach a steady-state traffic load. For each traffic load from 50 to 1000 Erlangs in steps of 50, and for arrival rates from 5 to 25 in steps of 5, we conduct 500 simulation trials with unique random seeds.  For each trial, we estimate the number of requests at which steady state is reached using the MSER-5 method \cite{franklin_stationarity_2008} (Marginal Standard Error Rule with batch size 5). We apply the MSER-5 method as it has been shown to be superior to other methods such as the mean crossing rule \cite{white_problem_2009}.

% \footnotetext{A blocking network reaches steady-state in less traffic requests than a non-blocking one, therefore we consider a non-blocking network to estimate an upper bound on the required warm-up period before steady state.}


% \subsubsection{Results and discussion}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{IMAGES/steady_state_boxplots.png}
%     \caption{No. of simulated requests necessary to reach the steady-state network traffic load specified on the x-axis, for a non-blocking network.}
%     \label{fig:traffic_warmup}
% \end{figure}

% Figure \ref{fig:traffic_warmup} displays results as box-and-whisker plots showing how many requests are needed to reach steady state for each traffic load. The whiskers extend to the most extreme data points within 1.5 times the inter-quartile range. We observe a linear relationship between traffic load and requests until steady state (warm-up period). We fit a line to the maximum values (tops of the whiskers) to determine the warm-up period with high confidence. The fitted line indicates that approximately 7 times the target traffic load in requests are required to reach steady state. Based on this finding, the 3000-request warm-up period used by DeepRMSA that we adopt in section \ref{sec:repro} is sufficient for our problem settings.



















\subsection{Holding time truncation}
\label{sec:holding_time}

In dynamic traffic simulations, the service holding time and time until the next arrival of a service request are modeled as exponentially distributed random variables, which is consistent with the assumption of Poisson arrival processes. Random sampling from these exponential distributions is used to generate specific times for each service request in the simulation.

DeepRMSA, Reward-RMSA, and GCN-RMSA use the same original DeepRMSA codebase as the basis for their experiments. This codebase includes a significant detail: the service holding time is resampled if the resulting value is more than twice the mean of the distribution. We refer to this detail as holding time truncation.  In order to recreate the problems from these papers, we analyze the effect of holding time truncation.


\subsubsection{Experiment setup}
To understand the effect of truncation on the traffic statistics, we define an exponential distribution with unit mean. We take $10^{6}$ samples from the distribution, both with and without truncation, and calculate the mean of the resulting sample populations in both cases.

\subsubsection{Results and discussion}
Figure \ref{fig:truncation} compares histograms of service holding times with and without truncation. The y-axis shows the probability density, which is normalized so the area of each histogram is one. The truncated case shows a cutoff at twice the mean holding time. The vertical lines indicate the mean holding time for each case.

Holding time truncation reduces the mean by approximately 31\%. This results in 31\% lower traffic load. Therefore, papers that use the DeepRMSA codebase (including DeepRMSA, Reward-RMSA, and GCN-RMSA) evaluate their solutions at traffic loads 31\% lower than reported. This detail is not made explicit in the published papers. This finding highlights the challenges in making fair comparisons between papers, and the need for transparency in research code.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{IMAGES/truncation.png}
    \caption{Histogram of service holding holding times. The truncated distribution resamples the holding time when the sampled value exceeds $2*$mean. This reduces the mean holding time by 31\% compared to the standard exponential distribution.}
    \label{fig:truncation}
\end{figure}



%Cisco NCS 2000 Flex Spectrum Single Module ROADM and it's integrated pre-amplifier has a nominal noise figure of 5.5dB (for 24dB gain) or 11.7dB (for 12dB gain), 















\subsection{Benchmarking of published results}
\label{sec:repro}
Our analysis of the best performing heuristics, of holding time truncation, and our correspondence with the authors enables us to benchmark the published results from the five selected influential papers. The aim of this comparison is to determine if any of the published RL solutions achieve lower SBP than the heuristics. %In order to do so, we recreate their simulations exactly and apply the KSP-FF heuristic algorithm with K=50 and paths ordered by number of hops in each case, based on our experiments from section \ref{sec:heuristic_comparison}.


\subsubsection{Experiment methodology}


We recreate the problems from each selected paper in our own simulation framework \cite{doherty_xlron_2024}. We match the topologies (NSFNET, COST239, JPN48, USNET), mean service arrival rates, mean service holding times, data-rate or bandwidth request distributions, and uniform traffic matrices. We use the same measurement methodology as described in the respective papers to reproduce results, which is 3000 request warm-up period (to allow the network blocking probability to reach steady-state after the 'initial transient' \cite{white_problem_2009}) followed by 10,000 requests. The SBP is calculated at the end of the episode. We run 10 independent episodes at each traffic load per problem and calculate the mean and standard deviation across trials.

We extract published results for KSP-FF and RL solutions from the papers, using textual values where available otherwise reading from charts. All published results report only a single data point for each traffic value, without uncertainty estimates. %We provide all of the extracted data and our results in Appendix \ref{appendix:A}.

We check that our results for KSP-FF with K=5 (green line in Figure \ref{fig:repro}) match the published results for KSP-FF (blue line in Figure \ref{fig:repro}) within two standard deviations to ensure faithful reproduction. This comparison gives us a high degree of confidence that we have exactly recreated each problem setting.



\subsubsection{Results and discussion}


\begin{figure*}[ht]
  \includegraphics[width=1.01\textwidth]{IMAGES/review_summary_plots_km.png}
  \caption{Mean SBP against traffic load. Each column is a publication and each subplot is for a topology. Error bars and shaded areas show standard deviations. %Data for $RL$ and 5-SP-FF$_{published}$ are extracted from the publications. Close agreement between 5-SP-FF$_{published}$ and  5-SP-FF$_{ours}$ show that we accurately reproduce each case of study.
  \mbox{50-SP-FF$_{hops}$} exceeds or matches the $RL$ performance for each case.}
  \label{fig:repro}
\end{figure*}

Figure \ref{fig:repro} shows our reproduction of results from the selected papers, with SBP against traffic load in Erlangs in each subplot. The plots are organized by paper (columns) and topology (rows). PtrNet-RSA has two columns reflecting its two test cases: networks with 40 FSU per link and 1 FSU requests, and networks with 80 FSU per link and 1-4 FSU requests. PtrNet-RSA only considers fixed-bandwidth requests (no distance-dependent modulation format). MaskRSA and PtrNet-RSA only consider single fibre links (counter-propagating channels) , whereas the other cases consider dual fibre links (one fibre for each direction of propagation), which increases their capacity.

Each plot contains 5 datasets:
\begin{itemize}[itemsep=0pt]
\item[] \textbf{RL}: Published results for the RL approach
\item[] \textbf{5-SP-FF$^{published}_{km}$}: Published results for KSP-FF (K=5) with paths ordered by \#km
\item[] \textbf{5-SP-FF$_{km}$}: Our results for KSP-FF (K=5) with paths ordered by \#km
\item[] \textbf{5-SP-FF$_{hops}$}: Our results for KSP-FF (K=5) with paths ordered by \#hops
\item[] \textbf{50-SP-FF$_{hops}$}: Our results for KSP-FF (K=50) with paths ordered by \#hops
\end{itemize}

Points show mean values, shaded areas indicate standard deviation and lines interpolate between points. The DeepRMSA paper provides data for only one traffic load per topology. The excellent agreement between 5-SP-FF$^{published}_{km}$ and 5-SP-FF$_{km}$ in all cases confirms that our framework accurately reproduces the published scenarios. %We can therefore make comparisons between our results on these problem settings and the published RL results with high confidence.


From Figure \ref{fig:repro}, we highlight the comparisons of 'RL' (red) with 5-SP-FF$_{hops}$ (orange), and 50-SP-FF$_{hops}$ (purple). 5-SP-FF$_{hops}$ reduces the blocking probability by up to an order of magnitude compared to RL in all cases for NSFNET, 4/5 cases for COST239 and 1/3 cases for USNET. This shows that ordering paths by \#hops is sufficient to beat the RL results in these cases.

For larger topologies, considering more candidate paths (K>5) improves the heuristic performance significantly, often by over an order of magnitude. As shown by Figure \ref{fig:repro}, 50-SP-FF$_{hops}$ gives the lowest SBP of all approaches in all cases, except PtrNet-RSA-80 USNET (bottom right).

For PtrNet-RSA-80 USNET, we consider it plausible that the pointer-net architecture is a contributing factor to the strong performance, as it is not limited to selecting from a pre-defined set of paths. However, as the published results in this case fall within one standard deviations of the mean for 50-SP-FF$_{hops}$, the result could be spurious. This highlights the need for summary statistics and confidence intervals from multiple trials to be included with published results.

In summary, the results show that making minor changes (ordering paths by \#hops and considering more paths)  to simple heuristic algorithms is sufficient to achieve lower blocking probability than the sophisticated RL solutions that have been published.

We highlight that this analysis, and the selected papers, focus on SBP as the optimization objective. In realistic scenarios, network blocking or throughput must be balanced with other metrics such as latency and total cost of operation from transceiver launch power, amplifiers, and other network elements. Future research should therefore focus on problems that take a holistic approach to network operations optimization with multiple objectives \cite{nallaperuma_interpreting_2023}, and incorporate sophisticated models of all physical layer effects for improved accuracy \cite{curri_gnpy_2022,buglia_closed-form_2023}.

%While our earlier experiments showed FF-KSP performs better than KSP-FF for JPN48, we only plot KSP-FF results as they already surpass the RL performance. For MaskRSA JPN48, FF-KSP with K=50 achieves zero blocking across all tested traffic loads.

% Could include a summary paragrph here and/or a note about how RL could do better but it needs to consider enough candidate paths and the set of candidate paths needs to prioritise those with less hops not just shorter distance.
%We note that it is theoretically possible for RL to equal or exceed the performance of the best heuristic algorithms. However, our results suggest that it is necessary to consider sufficiently diverse paths 

All data shown in Figure \ref{fig:repro} is provided in tabular form in Appendix A.



==> 2_PAPER_SECTIONS/6_network_blocking_bounds.tex <==
\section{Network blocking bounds}
\label{sec:bounds}

We have demonstrated in Section \ref{sec:repro_main} that many influential works on RL for DRA problems in optical networks have failed to improve on a simple heuristic algorithm. The extent to which it is possible to reduce the blocking probability, and increase supported traffic, is an important motivating factor in any future research into this topic. 

To understand the limits of blocking probability, we derive empirical lower bounds. By comparing these lower bounds to the performance of our best solution for a target SBP, we can estimate the additional traffic load that can be supported and, therefore, the maximum benefit from applying an intelligent resource allocation method such as RL. %We term this additional capacity the "optimality gap", as we consider our lower bound to be approximately optimal.

As discussed in section \ref{sec:background}, DRA problems in optical networks that require RSA are subject to three constraints: spectrum continuity, spectrum contiguity, and no reconfiguration. By relaxing any of these constraints, the optimal or near-optimal solution of the relaxed problem is a bound on the solution of the full problem. The cut-sets bound method of Cruzado et al \cite{cruzado_effective_2023,cruzado_capacity-bound_2024} relaxes the spectrum continuity constraint and uses insights from the min-cut max-flow theorem to estimate a lower bound SBP. We instead relax the constraint on reconfiguring already-established connections, a process known as defragmentation.

We couple this defragmentation with resource prioritization: sorting the active connection requests by their required resources and allocating them sequentially. The sorting of active requests in descending order of required resources was found to improve the achievable capacity to optimal or near-optimal by Baroni \cite{baroni_routing_1998} in static RWA and later Beghelli \cite{beghelli_resource_2006} for dynamic RWA, a method they refer to as 'reconfigurable routing'. Since our problem settings are elastic optical networks, we prefer the term defragmentation. The intuition behind this approach is to allocate higher-resource requests first so that requests with shorter paths and lower spectral requirements may be squeezed into remaining spectral gaps later.







\subsection*{Resource-Prioritized Defragmentation}
\label{sec:bounds}


\begin{algorithm}
\caption{Resource-Prioritized Defragmentation Blocking Bound Estimation}
\begin{algorithmic}[1]
\Require Network topology $G$, Set of requests $\mathcal{R}$, Frequency slots per link $F$
\Ensure Blocking probability $P_b$
\State $N \gets \textsc{InitializeNetwork}(G, F)$ \Comment{Initialize network state with empty spectrum slots}
\State $\textit{blocked} \gets \texttt{false}$
\State $\textit{blocked\_requests} \gets 0 $
\For{$t \gets 1$ to $|\mathcal{R}|$}
    \State $N \gets \textsc{RemoveExpiredRequests}(N, t)$
    \State $r_t \gets \textit{current request from } \mathcal{R}$
    \State $N$, $\textit{blocked} \gets \textsc{AllocateRequest}(N, r_t)$
    
    \If{$\textit{blocked}$}
        \State $\textit{active\_requests} \gets \textsc{GetActiveRequests}(\mathcal{R}, t)$
        \State $\textit{sorted\_requests} \gets \textsc{SortByResource}(\textit{active\_requests})$
        \State $N_{temp} \gets \textsc{InitializeNetwork}(G, F)$
        \State $\textit{blocked} \gets \texttt{false}$
        
        \For{$r \in \textit{sorted\_requests}$}
            \State $N$, $\textit{blocked} \gets \textsc{AllocateRequest}(N_{temp}, r)$
            \If{$\textit{blocked}$}
                \State \textbf{break}
            \EndIf
        \EndFor
        
        \If{not $\textit{blocked}$}
            \State $N \gets N_{temp}$
        \Else
            \State $\textit{blocked\_requests} \gets \textit{blocked\_requests} + 1$
        \EndIf
    \EndIf
\EndFor

\State \Return $\frac{\textit{blocked\_requests}}{|\mathcal{R}|}$
\end{algorithmic}
\label{algo:defrag}
\end{algorithm}

The resource-prioritized defragmentation algorithm is outlined in Algorithm \ref{algo:defrag}. It utilizes four key subroutines:

\begin{itemize}
    \item \textsc{RemoveExpiredRequests}($N$, $t$) maintains network state by removing connections that have expeired. For current time $t$, and request with arrival time $t_{\text{arrival}}$ and holding time $t_{\text{holding}}$, the expiry condition is defined as: $t_{\text{arrival}} + t_{\text{holding}} < t$.
    
    \item \textsc{AllocateRequest}($N$, $request$) establishes a new connection subject to continuity and contiguity constraints, and returns the updated network state and a boolean to indicate if the connection was blocked. We use the KSP-FF or FF-KSP algorithm with K=50. We select the algorithm that produces the lowest SBP for the problem instance.
    
    \item \textsc{GetActiveRequests}($\mathcal{R}$, $t$) identifies requests where $t_{\text{arrival}} \leq t < t_{\text{arrival}} + t_{\text{holding}}$, determining which connections require reallocation during defragmentation.
    
    \item \textsc{SortByResource}($requests$) orders active requests by required resources (product of required spectral slots and hops of shortest path), prioritizing larger requests during reallocation to maximize the probability of finding viable configurations.
    
\end{itemize}

A shortcoming of our method of blocking bound estimation is its reliance on the internal \textsc{AllocateRequest} heuristic. To have confidence that the solution presents a true bound, the allocation method must be as close to optimal as possible. We therefore evaluate multiple heuristics for each case, as shown in Section \ref{sec:heuristic_comparison}, and select the one with lowest SBP. We find the best performing heuristic is KSP-FF$_{hops}$ with K=50 for most cases, except MaskRSA JPN48 which is FF-KSP.


%Combined with resource prioritization (\textsc{SortByResource}) we assume the results are near-optimal, based on results from Baroni \cite{baroni_routing_1998}. 
An advantage of our method compared to cut-sets analysis is it computes an allocation that is guaranteed to be physically possible, as it relaxes the 'No Reconfiguration' constraint instead of the physical spectrum continuity constraint. Relaxing the 'No Reconfiguration' constraint makes Algorithm \ref{algo:defrag} omniscient (it has complete knowledge of requests to be allocated) rather than a strictly on-line algorithm, according to definitions from Awerbuch et al \cite{awerbuch_throughput-competitive_1993}. This gives Algorithm \ref{algo:defrag} a fundamental competitive advantage over on-line algorithms like KSP-FF/FF-KSP, therefore it can be considered a lower bound estimator of blocking probability. % This disparity in information may however mean it is too much of an upper-bound estimate
%Overall, resource-prioritized defragmentation bounds can be considered complimentary to cut-sets bounds due to the difference in constraint relaxation.

We note that our algorithm is general and can be applied to any DRA problem in optical networks by using a strong heuristic for \textsc{AllocateRequest} and defining the resource-based sort criteria appropriately.



\begin{figure*}[t]
  \includegraphics[width=1.01\textwidth]{IMAGES/bounds.png}
  \caption{Mean SBP against traffic load for the lowest-blocking heuristic in each case (KSP-FF or FF-KSP with K=50) and the estimated bound from Algorithm \ref{algo:defrag}. Each column is a publication and each subplot is for a topology. Shaded areas show standard deviations. Red lines and text indicate relative increase in supported traffic at 0.1\% SBP from heuristic to bound.}
  \label{fig:bounds}
\end{figure*}


\subsection{Experiment setup}

For each problem from the five selected papers, we run the best performing heuristic for a range of traffic loads that result in SBP from 0.01\% to 1\%. For the lowest-blocking heuristic and for Algorithm \ref{algo:defrag}, we run 10 episodes of 10,000 requests with unique random seeds and calculate the mean and standard deviation of SBP across episodes. We calculate the mean and standard deviation SBP across episodes in each case. 

We compare the resulting SBP from the best heuristic and from algorithm \ref{algo:defrag}. We seek to estimate the additional network capacity that can be achieved at 0.1\% SBP for each case of study from the five selected papers. We select 0.1\% SBP to align with previous studies of network throughput estimation by Cruzado et al \cite{cruzado_effective_2023,cruzado_capacity-bound_2024}.

\subsection{Results and discussion}


Similar to Figure \ref{fig:repro}, each subplot in Figure \ref{fig:bounds} represents a different problem instance. DeepRMSA, Reward-RMSA, and GCN-RMSA are combined into a single set of plots since they use identical topologies and traffic models. The purple lines show the best performing heuristic in each case (KSP-FF with K=50, or FF-KSP for JPN48), with paths sorted in ascending order of number of hops. The grey lines show the resource-prioritized defragmentation bounds. At 0.1\% SBP, we compare the network traffic loads that can be supported in each case, with the difference highlighted by a red horizontal line. The relative increase in network capacity is calculated as the difference between the upper bound traffic load and the heuristic traffic load, as a percentage of the heuristic load.

PtrNet-RSA-40 shows differences of 5\%, 1\%, and 8\% across its three test cases. These relatively low values are due to the fixed width requests size of 1 FSU used in this case, which makes it equivalent to RWA and reduces the impact of fragmentation compared to RSA/RMSA.

For the Deep/Reward/GCN-RMSA, MaskRSA and PtrNet-RSA-80 cases, the difference between the supported traffic in the heuristic case and the upper bound ranges from 19\% (MaskRSA JPN48) to 36\% (Deep/Reward/GCN-RMSA NSFNET). These results show larger but comparable optimality gaps to those from the cut-sets method of Cruzado et al. \cite{cruzado_capacity-bound_2024}, who found gaps of 5\% to 16\% in their cases of study. This shows that defragmentation can unlock significant network capacity, but it is unknown theoretically how close an intelligent online allocation method, such as RL, can come to this bound. This will be the subject of future research.


==> 2_PAPER_SECTIONS/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


Our review of the field of RL applied to DRA problems in optical networks shows that it has been the subject of significant research interest, with almost 100 peer-reviewed papers published so far. Technical innovations from ML research, such as invalid action masking \cite{shimoda_mask_2021,nevin_techniques_2022,cheng_ptrnet-rsa_2024} and GNNs \cite{xu_deep_2022,li_gnn-based_2022,xiong_graph_2024}, have been applied to the problem area and have demonstrated incremental improvements in network blocking.

However, the field has suffered from a lack of standardization in problems, selective application of benchmark algorithms, and poor practices for reproducibility. We have addressed these problems by assessing a range of heuristic algorithms, optimizing their path ordering and number of candidate paths, and applying them to the problem settings from five influential papers on RL for DRA. We use our simulation framework for this work, which enabled recreation of diverse problem settings and fast computation.

From our assessment and optimization of heuristic algorithms, we determine that KSP-FF or FF-KSP with K=50 are generally the best available. We highlight the result that ordering the pre-computed shortest paths by number of hops gives significantly lower blocking probability than ordering by distance. These benchmarking recommendations can be applied to future studies of RL or other solution methods.

 %Our quantification of the effects on mean path length of reordering paths in this way show that the mean length is increased by around 20\% in most cases, which is likely an acceptable trade-off in exchange for greater network capacity. %We also quantify the effect of network warm-up, and make recommendations that the warm-up period should be at least 7x the target traffic load to allow stabilization before training or evaluating on dynamic network traffic.

Our most significant findings are in the benchmarking of previous RL results. By extracting the published results of RL from the selected papers, and comparing to the best heuristic benchmarks on recreated problem settings, we show that simple heuristics can exceed or match RL in all cases, often with over an order of magnitude lower SBP. This shows the relative performance of RL on these problems has been overestimated due to weak benchmarks, and highlights the need for more rigorous standards of evaluation on these problems to avoid trivial results. These standards also apply to other non-RL resource allocation algorithms.

Finally, to ascertain the practical value of pursuing further research into optimized DRA, we provide the Resource-Prioritized Defragmentation method of estimating the lower bound network blocking probability. Compared to the best heuristics available for each case, this method estimates the upper bound additional dynamic traffic load that can be supported on flex-grid networks is approximately 19\% to 36\%. These results suggest there is room for improvement over the best benchmarks, which may motivate further research into DRA with RL or other methods. Alternatively, research into network optimization with RL could focus on other objectives for which there are not yet good heuristic solutions.


%Considering that IP traffic is projected to increase at approximately 20\% annually until 2029 \cite{ericsson_ab_ericsson_2024}, it is an open question if the potential percentage gains in network throughput are worth pursuing with RL, or if research into network optimization with RL should focus on other objectives for which there are not yet good heuristic solutions.


% Our method of capacity bound estimation is simple and scalable, and can be used by other researchers to estimate the quality of their solution. It is also adaptable to other DRA problems

% We show 2 important qunatitative results. 1) Heuristics give lower service blocking probability than Rl for all published works. 2)


==> 2_PAPER_SECTIONS/results_table.tex <==
%\onecolumn
%\centering
%\scriptsize

\newpage
\onecolumn
\appendix
\section{Appendix: Data from previous works and our benchmarks}
\label{appendix:A}
\nopagebreak
\setlength{\tabcolsep}{6pt}


\begin{longtable}[!htbp]{llll|lllll|l}

\caption*{Comparison of service blocking probabilities for KSP-FF and RL solutions across various topologies and traffic loads.}\label{tab:blocking_probabilities} \\
\hline
\multirow{3}{*}{\textbf{Publication}} & \multirow{3}{*}{\textbf{Topology}} & \multirow{3}{*}{\textbf{N$_{slots}$}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Load \\ (Erlang)\end{tabular}}} & \multicolumn{5}{c|}{\textbf{Service blocking probability (\%)}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mean \\ improvement \\ over RL (\%)\end{tabular}}} \\
\cline{5-9}
 &  &  &  & \multicolumn{2}{c|}{Published} & \multicolumn{3}{c|}{Ours} &  \\
\cline{5-9}
 &  &  &  & RL & \multicolumn{1}{c|}{5-SP-FF} & 5-SP-FF & 5-SP-FF$_{hops}$ & 50-SP-FF$_{hops}$ &  \\
\hline
\endfirsthead

\multicolumn{10}{c}{continued from previous page} \\
\hline
\multirow{3}{*}{\textbf{Publication}} & \multirow{3}{*}{\textbf{Topology}} & \multirow{3}{*}{\textbf{N$_{slots}$}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Load \\ (Erlang)\end{tabular}}} & \multicolumn{5}{c|}{\textbf{Service blocking probability (\%)}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mean \\ improvement \\ over RL (\%)\end{tabular}}} \\
\cline{5-9}
 &  &  &  & \multicolumn{2}{c|}{Published} & \multicolumn{3}{c|}{Ours} &  \\
\cline{5-9}
 &  &  &  & RL & \multicolumn{1}{c|}{5-SP-FF} & 5-SP-FF & 5-SP-FF$_{hops}$ & 50-SP-FF$_{hops}$ & \\
\hline
\endhead

\hline
\multicolumn{10}{r}{Continued on next page} \\
\endfoot

\hline
\endlastfoot

DeepRMSA             & NSFNET            & 100                  & 250                                                               & 4.00    & \multicolumn{1}{l|}{5.10}     & 5.00 ± 0.29 & 2.93 ± 0.22      & 2.33 ± 0.25                  & 42                                                                                    \\
DeepRMSA             & COST239           & 100                  & 600                                                               & 5.75 & \multicolumn{1}{l|}{6.75}    & 6.69 ± 0.35  & 3.80 ± 0.39      & 2.61 ± 0.36                  & 55                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 168                                                               & 0.35  & \multicolumn{1}{l|}{1.00}       & 1.06 ± 0.11  & 0.10 ± 0.02      & 0.02 ± 0.01                  & 94                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 182                                                               & 0.70  & \multicolumn{1}{l|}{1.40}       & 1.53 ± 0.15  & 0.25 ± 0.03      & 0.08 ± 0.03                  & 89                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 196                                                               & 1.20  & \multicolumn{1}{l|}{2.10}       & 2.06 ± 0.12  & 0.48 ± 0.07      & 0.21 ± 0.04                  & 83                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 210                                                               & 1.80  & \multicolumn{1}{l|}{2.70}       & 2.68 ± 0.20 & 0.95 ± 0.11      & 0.47 ± 0.05                  & 74                                                                                    \\                                                      
GCN-RMSA             & NSFNET            & 100                  & 154                                                               & 0.51 & \multicolumn{1}{l|}{0.67}    & 0.69 ± 0.08 & 0.03 ± 0.02      & 0.01 ± 0.00                  & 98                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 168                                                               & 0.66 & \multicolumn{1}{l|}{1.00}       & 1.06 ± 0.11 & 0.10 ± 0.02      & 0.02 ± 0.01                  & 97                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 182                                                               & 0.98 & \multicolumn{1}{l|}{1.42}    & 1.53 ± 0.15 & 0.25 ± 0.03      & 0.08 ± 0.03                  & 92                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 196                                                               & 1.50  & \multicolumn{1}{l|}{2.10}     & 2.06 ± 0.12 & 0.48 ± 0.07      & 0.21 ± 0.04                  & 86                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 210                                                               & 2.10  & \multicolumn{1}{l|}{2.76}    & 2.68 ± 0.20 & 0.95 ± 0.11      & 0.47 ± 0.05                  & 78                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 368                                                               & 0.71 & \multicolumn{1}{l|}{0.78}    & 0.80 ± 0.08 & 0.07 ± 0.03      & 0.00 ± 0.00                  & 100                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 391                                                               & 0.85 & \multicolumn{1}{l|}{1.30}     & 1.13 ± 0.12    & 0.17 ± 0.07      & 0.00 ± 0.00                  & 100                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 414                                                               & 1.25 & \multicolumn{1}{l|}{1.70}     & 1.57 ± 0.13 & 0.28 ± 0.09      & 0.01 ± 0.01                  & 100                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 437                                                               & 1.75 & \multicolumn{1}{l|}{2.30}     & 2.02 ± 0.13 & 0.46 ± 0.11      & 0.02 ± 0.02                  & 99                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 460                                                               & 2.10  & \multicolumn{1}{l|}{2.70}     & 2.53 ± 0.21 & 0.73 ± 0.20      & 0.07 ± 0.03                  & 97                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 320                                                               & 0.65 & \multicolumn{1}{l|}{0.75}    & 0.98 ± 0.10 & 0.25 ± 0.07      & 0.00 ± 0.01                  & 100                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 340                                                               & 0.83 & \multicolumn{1}{l|}{1.20}     & 1.31 ± 0.16 & 0.42 ± 0.07      & 0.01 ± 0.02                  & 99                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 360                                                               & 1.05 & \multicolumn{1}{l|}{1.50}     & 1.69 ± 0.12 & 0.73 ± 0.16      & 0.04 ± 0.04                  & 96                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 380                                                               & 1.60  & \multicolumn{1}{l|}{2.15}    & 2.18 ± 0.19 & 1.05 ± 0.19      & 0.09 ± 0.09                  & 94                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 400                                                               & 2.20  & \multicolumn{1}{l|}{2.70}     & 2.79 ± 0.24 & 1.53 ± 0.18      & 0.23 ± 0.09                  & 90                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 80                                                                & 0.01 & \multicolumn{1}{l|}{0.26}    & 0.33 ± 0.06 & 0.00 ± 0.00      & 0.00 ± 0.00                  & 100                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 90                                                                & 0.05 & \multicolumn{1}{l|}{0.60}     & 0.64 ± 0.07 & 0.01 ± 0.01      & 0.00 ± 0.00                  & 100                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 100                                                               & 0.20  & \multicolumn{1}{l|}{0.90}     & 1.08 ± 0.10 & 0.08 ± 0.05      & 0.04 ± 0.02                  & 80                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 110                                                               & 0.50  & \multicolumn{1}{l|}{1.80}     & 1.68 ± 0.11 & 0.25 ± 0.09      & 0.13 ± 0.03                  & 74                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 120                                                               & 0.79 & \multicolumn{1}{l|}{2.47}    & 2.39 ± 0.14 & 0.60 ± 0.14      & 0.33 ± 0.12                  & 58                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 130                                                               & 1.80  & \multicolumn{1}{l|}{3.00}       & 3.14 ± 0.22 & 1.35 ± 0.12      & 0.86 ± 0.14                  & 52                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 140                                                               & 3.00    & \multicolumn{1}{l|}{4.00}       & 4.05 ± 0.21 & 2.26 ± 0.23      & 1.71 ± 0.27                  & 43                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 150                                                               & 4.30  & \multicolumn{1}{l|}{5.00}       & 5.19 ± 0.28 & 3.43 ± 0.21      & 2.84 ± 0.26                  & 34                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 160                                                               & 5.30  & \multicolumn{1}{l|}{6.00}       & 6.37 ± 0.26 & 4.65 ± 0.35      & 4.15 ± 0.27                  & 22                                                                                    \\
MaskRSA              & JPN48             & 80                   & 120                                                               & 0.05 & \multicolumn{1}{l|}{1.60}     & 1.92 ± 0.27 & 0.32 ± 0.08      & 0.00 ± 0.00                  & 100                                                                                    \\
MaskRSA              & JPN48             & 80                   & 130                                                               & 0.20  & \multicolumn{1}{l|}{2.50}     & 2.75 ± 0.31 & 0.64 ± 0.10      & 0.02 ± 0.01                  & 90                                                                                    \\
MaskRSA              & JPN48             & 80                   & 140                                                               & 0.55 & \multicolumn{1}{l|}{3.50}     & 3.69 ± 0.30 & 0.97 ± 0.14      & 0.04 ± 0.03                  & 93 \\
MaskRSA              & JPN48             & 80                   & 150                                                               & 0.90  & \multicolumn{1}{l|}{4.50}     & 4.55 ± 0.32 & 1.41 ± 0.15      & 0.09 ± 0.04                  & 90                                                                                    \\
MaskRSA              & JPN48             & 80                   & 160                                                               & 1.60  & \multicolumn{1}{l|}{5.00}       & 5.40 ± 0.36 & 2.00 ± 0.21      & 0.18 ± 0.04                  & 89                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 180                                                               & 0.01 & \multicolumn{1}{l|}{0.80}     & 0.93 ± 0.11 & 0.00 ± 0.00      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 190                                                               & 0.03 & \multicolumn{1}{l|}{1.25}    & 1.27 ± 0.10 & 0.01 ± 0.01      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 200                                                               & 0.08 & \multicolumn{1}{l|}{1.50}     & 1.68 ± 0.10 & 0.02 ± 0.01      & 0.00 ± 0.01                  & 100                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 210                                                               & 0.19 & \multicolumn{1}{l|}{1.90}     & 2.06 ± 0.11 & 0.09 ± 0.04      & 0.03 ± 0.02                  & 84                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 220                                                               & 0.23 & \multicolumn{1}{l|}{2.50}     & 2.58 ± 0.11 & 0.22 ± 0.09      & 0.09 ± 0.05                  & 61                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 230                                                               & 0.75 & \multicolumn{1}{l|}{2.90}     & 3.14 ± 0.14 & 0.48 ± 0.12      & 0.26 ± 0.10                  & 65                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 240                                                               & 1.30  & \multicolumn{1}{l|}{3.50}     & 4.01 ± 0.22 & 0.90 ± 0.18      & 0.54 ± 0.15                  & 58                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 340                                                               & 0.01 & \multicolumn{1}{l|}{2.50}     & 3.36 ± 0.16 & 0.02 ± 0.02      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 360                                                               & 0.04 & \multicolumn{1}{l|}{3.25}    & 4.02 ± 0.20  & 0.04 ± 0.02      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 380                                                               & 0.12 & \multicolumn{1}{l|}{3.80}     & 4.72 ± 0.29 & 0.10 ± 0.03      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 400                                                               & 0.24 & \multicolumn{1}{l|}{4.60}     & 5.43 ± 0.36 & 0.25 ± 0.09      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 420                                                               & 0.39 & \multicolumn{1}{l|}{5.50}     & 6.24 ± 0.25 & 0.46 ± 0.12      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 210                                                               & 0.01 & \multicolumn{1}{l|}{0.85}    & 1.02 ± 0.20 & 0.14 ± 0.05      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 220                                                               & 0.08 & \multicolumn{1}{l|}{1.40}     & 1.46 ± 0.25 & 0.29 ± 0.08      & 0.00 ± 0.01                  & 100                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 230                                                               & 0.22 & \multicolumn{1}{l|}{1.85}    & 1.99 ± 0.31 & 0.46 ± 0.10      & 0.02 ± 0.01                  & 91                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 240                                                               & 0.38 & \multicolumn{1}{l|}{2.20}     & 2.59 ± 0.38 & 0.77 ± 0.18      & 0.08 ± 0.06                  & 79                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 250                                                               & 0.68 & \multicolumn{1}{l|}{3.10}     & 3.25 ± 0.32 & 1.19 ± 0.28      & 0.19 ± 0.09                  & 72                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 260                                                               & 1.10  & \multicolumn{1}{l|}{3.60}     & 3.87 ± 0.49 & 1.81 ± 0.35      & 0.42 ± 0.15                  & 62                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 270                                                               & 1.80  & \multicolumn{1}{l|}{4.40}     & 4.67 ± 0.50 & 2.39 ± 0.41      & 0.72 ± 0.27                  & 60                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 280                                                               & 2.20  & \multicolumn{1}{l|}{4.90}     & 5.40 ± 0.46 & 3.16 ± 0.48      & 1.25 ± 0.34                  & 43                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 200                                                               & 0.01 & \multicolumn{1}{l|}{0.60}     & 0.61 ± 0.09 & 0.00 ± 0.00      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 210                                                               & 0.03 & \multicolumn{1}{l|}{0.80}     & 0.83 ± 0.10 & 0.00 ± 0.00      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 220                                                               & 0.11 & \multicolumn{1}{l|}{1.20}     & 1.07 ± 0.09 & 0.02 ± 0.02      & 0.01 ± 0.02                  & 91                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 230                                                               & 0.16 & \multicolumn{1}{l|}{1.40}     & 1.32 ± 0.13 & 0.05 ± 0.03      & 0.02 ± 0.02                  & 88                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 240                                                               & 0.50  & \multicolumn{1}{l|}{1.90}     & 1.63 ± 0.15 & 0.11 ± 0.06      & 0.05 ± 0.04                  & 90                                                                                    \\
PtrNet-RSA           & COST239           & 80                   & 420                                                               & 0.01 & \multicolumn{1}{l|}{2.50}     & 2.66 ± 0.11  & 0.08 ± 0.03      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & COST239           & 80                   & 440                                                               & 0.16 & \multicolumn{1}{l|}{3.00}       & 3.05 ± 0.16 & 0.13 ± 0.06      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & COST239           & 80                   & 460                                                               & 0.65 & \multicolumn{1}{l|}{3.50}     & 3.52 ± 0.19 & 0.25 ± 0.07      & 0.01 ± 0.01                  & 98                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 260                                                               & 0.03 & \multicolumn{1}{l|}{1.00}       & 1.21 ± 0.18 & 0.46 ± 0.13      & 0.00 ± 0.00                  & 100                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 270                                                               & 0.09 & \multicolumn{1}{l|}{1.20}     & 1.48 ± 0.24 & 0.64 ± 0.18      & 0.16 ± 0.09                  & -78                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 280                                                               & 0.15 & \multicolumn{1}{l|}{1.40}     & 1.78 ± 0.20 & 0.87 ± 0.21      & 0.38 ± 0.13                  & -153                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 290                                                               & 0.29 & \multicolumn{1}{l|}{1.70}     & 2.13 ± 0.24 & 1.12 ± 0.24      & 0.54 ± 0.15                  & -86                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 300                                                               & 0.52 & \multicolumn{1}{l|}{2.20}     & 2.46 ± 0.23 & 1.42 ± 0.29      & 0.61 ± 0.20                  & -33                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 310                                                               & 0.66 & \multicolumn{1}{l|}{2.40}     & 2.79 ± 0.26 & 1.75 ± 0.32      & 0.88 ± 0.23                  & -33                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 320                                                               & 1.00    & \multicolumn{1}{l|}{2.80}     & 3.18 ± 0.31 & 2.08 ± 0.35      & 1.15 ± 0.26                  & -15                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 330                                                               & 1.50  & \multicolumn{1}{l|}{3.10}     & 3.50 ± 0.28 & 2.42 ± 0.31      & 1.46 ± 0.30                  & 3                                                                                    
\end{longtable}

==> archive/3_literature_survey.tex <==
\section{Literature Survey}
\label{sec:survey}

There exists a considerable body of literature on RL for dynamic resource allocation (DRA) in optical networks \cite{amin_survey_2021}. DRA in optical networks is distinguished from similar problems in electronically linked networks by the nature of fibre optic links. The capacity of each fibre link is a vector of available wavelengths or spectrum slots, as defined by the ITU standards G.671 and G.694.2 \cite{international_telecommunication_union_spectral_2002,international_telecommunication_union_transmission_2012}, not a scalar quantity. Due to this fundamental difference, we only consider publications related to optical networks in this review, but acknowledge the closely related body of literature on RL for other graph-based resource allocation problems.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{IMAGES/RL_RSA_litreview_barchart.png}
    \caption{Count of publications related to RL for DRA problems in optical networks. Citations for each classification category are: RWA \cite{garcia_multicast_2003,pointurier_reinforcement_2007,koyanagi_reinforcement_2009,suarez-varela_routing_2019,shiraki_dynamic_2019,shiraki_reinforcement-learning-based_2019,zhao_cost-efficient_2021,freire-hermelo_dynamic_2021,liu_waveband_2021,nevin_techniques_2022,di_cicco_deep_2022,di_cicco_deepls_2023,nallaperuma_interpreting_2023}, RSA \cite{reyes_adaptive_2017,li_deepcoop_2020,li_multi-objective_2020,wang_dynamic_2021,zhao_reinforced_2021,shimoda_deep_2021,shimoda_mask_2021,romero_reyes_towards_2021,zhao_rsa_2022,wu_service_2022,arce_reinforcement_2022,quang_magc-rsa_2022,cruzado_reinforcement-learning-based_2022,jiao_reliability-oriented_2022,hernandez-chulde_experimental_2023,sharma_deep_2023,lin_deep-reinforcement-learning-based_2023,tanaka_pre-_2023,cheng_ptrnet-rsa_2024}, RMSA \cite{chen_deeprmsa_2019,luo_leveraging_2019,chen_multi-task-learning-based_2021,shi_deep-reinforced_2021,sheikh_multi-band_2021,xu_spectrum_2021,gonzalez_improving_2022,tang_deep_2022,momo_ziazet_deep_2022,terki_routing_2022,tu_entropy-based_2022,cheng_routing_2022,xu_deep_2022,pinto-rios_resource_2022,tang_heuristic_2022,luo_survivable_2022,sadeghi_performance_2023,errea_deep_2023,terki_routing_2023,tang_routing_2023,xu_hierarchical_2023,li_opticgai_2024,teng_drl-assisted_2024,teng_deep-reinforcement-learning-based_2024}, Other \cite{boyan_packet_1993,ma_demonstration_2019,zhao_reinforcement-learning-based_2019,wang_subcarrier-slot_2019,natalino_optical_2020,ma_co-allocation_2020,weixer_reinforcement_2020,wang_deepcms_2020,tian_reconfiguring_2021,liu_multi-agent_2021,zhao_service_2021,morales_multi-band_2021,hernandez-chulde_evaluation_2022,koch_reinforcement_2022,tanaka_reinforcement-learning-based_2022,etezadi_deepdefrag_2022,beghelli_approaches_2023,renjith_deep_2023,davalos_triggering_2023,etezadi_deep_2023,zhang_admire_2023,tanaka_adaptive_2023,johari_drl-assisted_2023,pavon-marino_tree-determination_2023,fan_blocking-driven_2023,yin_dnn_2024,li_tabdeep_2024,tanaka_reinforcement-learning-based_2024,lian_dynamic_2024,doherty_xlron_2024,wang_availability-aware_2024,tse_reinforcement_2024,jara_dream-gym_2024}.}
    \label{fig:lit_barchart}
\end{figure}



\subsection{Survey methodology}
\label{sec:survey-methodology}

To find relevant papers, we searched the Google Scholar database using the following search terms: "'REINFORCEMENT LEARNING' AND 'NETWORK' AND ('OPTICAL' OR 'WAVELENGTH' OR 'SPECTRUM')". Papers were limited to English-language peer-reviewed articles. We filtered the search results by inspection of paper titles and abstracts, and manually added any related works from our own citation database that were missing from the initial search. A review of the collected papers then created the final set of 96.

We reviewed each paper in the set to classify them into four broad categories: 'RWA', 'RSA', 'RMSA' for those that apply RL to the respective problem variants, and 'Other'.
The 'Other' category includes papers that are concerned with RL applied to: traffic grooming, defragmentation, survivability or service restoration, multicast provisioning, simulation training environments, and other problem variants such as transceiver parameter optimisation.

We notice the following characteristics and trends in the gathered dataset of papers: 
1) Increase in papers from 2019 onwards due to DeepRMSA seminal paper. Arrival of paper in 2019 shows time lag between cutting edge ML papers (Atari in 2013 and AlphaGo 2016) and adoption of techniques by optical networks research community.
2) RWA occupied large proportion of total papers in 2019 and before but became a smaller proportion and no publications in 2024.
3) 2020 impact of COVID pandemic on total publications
4) Peak in interest in 2022
5) More physically realistic and relevant problem, RMSA, has grown compared to RWA and RSA.
6) Proportion of Other has grown despite overall decline in publication count. We hypothesise this is due to saturation of results in the field and lack of breakthrough performance, while attention has shifted to more novel problems. 


% TODO - Include graphic showing filtering methodology
% What about a timeline of developments on RL and RL-applied-to-RSA? Would be good to highlight the 






\subsection{Early applications of RL to RSA}
\label{sec:survey-early_applications}

The first application of RL to network routing (in a packet switched network) was in 1993 \cite{boyan_packet_1993}, which used Q-learning to continuously update a routing table for a 6x6 network. The optical networks community later picked up the technique in 2003 when Garcia et al investigated RL for multicast in WDM networks \cite{garcia_multicast_2003}. We note that multiple works then considered routing in Optical Burst Switched networks due to the research interest in that emerging networking paradigm at the time \cite{kiran_reinforcement_2006,belbekkouche_reinforcement_2008}. Koyanagi also \cite{koyanagi_reinforcement_2009} employed Q-learning for the task of service differentiation and noted the algorithm's sensitivity to hyperparameter selection. 

A significant milestone was then achieved by the work of Pointurier and Heidari \cite{pointurier_reinforcement_2007}, which used the simple RL technique "Linear Reward-$\epsilon$ Penalty" (LR$\epsilon$P) to update a routing table for a WDM network while accounting for quality of transmission (QoT) constraints, showing lower blocking probability than Shortest Path (SP) routing. This paper was the first to consider dynamic network traffic and to demonstrate improvement over a widely used heuristic, although it neglected to consider KSP-FF. 

A decade later in in 2017, Reyes amd Bauschert \cite{reyes_adaptive_2017} were the first to consider the problem of dynamic traffic in flex-grid networks, again using a Q-table technique. The modern era of RL, using deep neural networks as function approximators for Q-tables, was widely established by 2013 with the publication of results from Deepmind on RL for Atari videogames \cite{mnih_asynchronous_2016}. These more advanced techniques then began to be applied in optical networks in 2018, when the original DeepRMSA paper was presented at Optical Fibre Communications Conference. This seminal paper then spurred a series of incremental advances published from 2019 onwards.




\subsection{DeepRMSA and successor works}
\label{sec:survey-deeprmsa}

DeepRMSA \cite{chen_deeprmsa_2019} is the most influential paper in the field RL for DRA problems on optical networks. It's notable for being the first paper to achieve lower blocking probability than KSP-FF, through its use of a multi-layer perceptron (MLP) neural network as a function approximator for the learned policy, and its feature engineering of the observation space to enable more efficient learning. This success sparked a series of successor works.

We define successor works as papers that (i) use DeepRMSA as a benchmark, and (ii) show evidence of using the DeepRMSA codebase. Most published works do not make their code publicly available, however DeepRMSA is notable in providing open source code. Consequently, this has been used by other researchers and implementation details found in the DeepRMSA codebase have propagated to other works but not been made explicit in publications. The esoteric implementation details that originate in the DeepRMSA codebase are (i) network warm-up period, and (ii) truncated service holding time. We quantify the effects of both of these details in section \ref{sec:empirical_analysis}.

The direct successor works are from Chen et al using the DeepRMSA framework with transfer learning on different topologies and traffic \cite{chen_multi-task-learning-based_2021}, Tang et al using a shaped reward function to improve performance, Xu et al using graph and recurrent neural networks to for the policy network to improve performance \cite{xu_deep_2022}, Xu et al investigate a hierarchical framework for multi-domain networks \cite{xu_hierarchical_2023}, Errea et al use DeepRMSA with two choices of first slots per path \cite{errea_deep_2023}. DeepRMSA has also been used as a benchmark in MaskRSA \cite{shimoda_mask_2021} and PtrNet-RSA \cite{cheng_ptrnet-rsa_2024}.



\subsection{Function approximation and neural network architectures}
\label{sec:survey-function_approximators}

Optic-GAI \cite{li_opticgai_2024} uses a diffusion model, a generative model based on an iterative de-noising process and most often applied to image synthesis \cite{ho_denoising_2020}, as represent the RWA policy. This allows 

\cite{suarez-varela_routing_2019} \cite{suarez-varela_graph_2023} \cite{li_gnn-based_2022} \cite{cheng_ptrnet-rsa_2024}


\subsection{Hyperparameter evaluation}

\cite{suarez-varela_routing_2019} is the first work to actually tune hyperparameters. \cite{chen_deeprmsa_2019} made some nod towards optimisation. Many papers simply compare 



\subsection{Invalid action masking for RSA}
\label{sec:survey-masking}




\subsection{Physical layer models}
\label{sec:survey-physical_layer}
QoT-aware papers
% Most studies of the problem make simplifying assumptions about the physical layer, e.g. calculating the maximum reach of each available modulation format by making worst-case assumptions on link occupancy and resulting non-linear effects. 


Notes on PtrNet-RSA:
\textbf{Claims:} 
\textbf{Limitations:} It appears to consider a directed graph with 


\subsection{Traffic models}
\label{sec:survey-traffic_models}

\subsection{Traffic Grooming}
\label{sec:survey-grooming}


\subsection{Problem variants}
\label{sec:survey-problem_variants}
 
\textbf{Multiband}

\textbf{Multicore}

\textbf{Defragmentation} Defragmentation is outside of the scope of this work and is unlikely to be adopted by network operators.

\textbf{Other} For completeness, we mention other problem variants here. Tidal optical networks, scheduling, defragmentation, etc.

RWA with power allocation recently explored by Tse et al \cite{tse_reinforcement_2024} uses 



\subsection{Network capacity bound estimation}
\label{sec:survey-capacity_bounds}

% Comment from Robin: Really baroni should be the starting point here and david ives also has work that looks at the limiting cut which is 5-6 years before this

\cite{hayashi_efficient_2022} - first BV-VDL paper.

\cite{hayashi_cost-effective_2023} - This paper introduced the concept of cut-sets analysis on optical networks to identify congested links. Cut set analysis originates from the study of packet switched networks. Cruzado et al modify the technique to apply to the spectrum-based connections on optical networks.

\cite{cruzado_effective_2023} - Proposes cut-sets method to estimate network capacity for fixed-grid RWA and suggests heuristic algorithm for RSA that incorporates this information.

\cite{cruzado_capacity-bound_2024} - Proposes cut-sets method to estimate network capacity for flex-grid elastic optical network with distance-adaptive modulation format. 

% Do we also need to include e.g. AUR-E here? 



\subsection{Reporting metrics}
To conclude the survey of the literature, the reporting metrics 
Use bitrate blocking probability instead of service blocking probability, especially if traffic requests have diverse bitrate requirements.
Target metric - set a target bitrate blocking probability and the \% improvement reported is in the increased traffic level that can be supported at the target blocking probability.


\subsection{Robustness of results}
Problems with the number of trials (not a statistically significant number of blocking events in many cases) and no uncertainty estimates are published.
Comparison to other RL solutions is not fair as the final performance depends greatly on the training regime. If the problem setting changes from that in the original paper for an RL solution, then hyperparameters must be re-tuned (rather than relying on published values). Even the random seed for the training run can affect the outcome, and to be fair a range of seeds e.g. 5 minimum should be used in order to have a range of values and compare against the maximum performance. Simply put, it is not meaningful to compare against another RL solution unless a comparable or reasonable amount of computing resources have been spent on tuning hyperparameters and training the final model, as were spent on the novel proposal.
Lack of open source to verify results.


==> archive/4_empirical_analysis.tex <==
\section{Empirical Analysis}
\label{sec:empirical_analysis}

To analyze the progress made in applications of RL to DRA problems in optical networks, we select 5 influential papers from the literature. Following our review of the field in section \ref{sec:survey}, we select these papers based on the criteria of influence (measured by citation count), novelty, and performance relative to benchmarks. The comparison of the papers is facilitated by their common problem settings (RSA/RMSA), topologies (NSFNET, COST239, USNET), and target metric (service blocking probability). We choose to focus on RSA/RMSA because they are the most widely studied DRA problems in the context of optical networks and they form a core sub-task of any other DRA problems on optical networks, such as VNF or VONE. Understanding RL performance on RSA/RMSA therefore has implications for the study of more complex problems.

In this section, we first summarize the selected papers, highlighting their novelty and contributions. Then, to decide on our benchmark heuristics, we compare six heuristics from the literature on a range of network topologies, traffic loads, and number of pre-calculated shortest paths.  We also provide analysis of simulation settings that affect the network blocking probability but have not previously been discussed in detail; network warm-up period, service holding time truncation, and path prioritization. We then present the results of our reproduction of the cases of study, which account for these effects, and compare to the best heuristics for each case, which show superior performance to all of the published RL solutions.

We conclude the section by explaining our methodology for estimating network capacity bounds, and present those bounds in comparison to our improved heuristic results. We provide all the scripts to reproduce our experiments and figures at the code repository for this work \cite{michael_doherty_micdohxlron_2024}.
%The bounds are found to be very close to the heuristic performance, which raises the question of how worthwhile RL solutions are for this class of DRA problems.

We use XLRON for all simulations \cite{doherty_xlron_2023}. It has demonstrated 10x faster training on CPU and over 1000x faster when parallelized on GPU compared to optical-rl-gym. This is possible due to its simplified data model and its implementation using the JAX high-performance array computing framework, that enables just-in-time compilation to accelerator hardware. It also offers a complete suite of unit tests for core functionality, therefore is more reliable than other libraries. We use it for these reasons and for its simple command-line interface, for ease of reproducibility and experiment automation.











\subsection{Summaries of selected papers}
\label{sec:paper_summaries}


\begin{enumerate}
    \item \textbf{DeepRMSA} \cite{chen_deeprmsa_2019} is the seminal paper in the field of RL for RMSA, with over 127 citations. It constructs a feature matrix to represent the available paths for the current requests and applies a simple MLP with 5 x 128 hidden units to select from the k-shortest paths with first-fit spectrum allocation. It demonstrates improved performance over KSP-FF on the NSFNET and COST239 topologies. DeepRMSA's impact was enhanced by releasing its codebase as open source.
    \item \textbf{Reward-RMSA} \cite{tang_heuristic_2022}, with over 15 citations, builds on the DeepRMSA framework and changes the reward function to incorporate fragmentation-related information. They demonstrate improvement over heuristics and their implementation of DeepRMSA.
    \item \textbf{GCN-RMSA} \cite{xu_deep_2022} has over 24 citations and is notable because it is the first work to use advanced neural network architectures to improve performance. They use a graph convolutional network (GCN) (including recurrent neural network (RNN) as the path aggregation function) in the policy and value functions, which they claim allows improved feature extraction from the network state. Like DeepRMSA and Reward-RMSA, the policy selects from K paths with first-fit spectrum allocation. They perform a thorough analysis of their proposed solution, showing improvement over benchmarks DeepRMSA and KSP-FF on the NSFNET, COST239, and USNET topologies. 
    \item \textbf{MaskRSA} \cite{shimoda_mask_2021} has over 25 citations. It innovated by selecting from the entire range of available slots on the K paths and using invalid action masking \cite{huang_closer_2020} to increase the efficiency of training. Despite the RSA in the title, the paper does consider distance-dependent modulation format. MaskRSA presented improvements over KSP-FF on the NSFNET and JPN48 topologies with over an order of magnitude lower blocking probability, or a 35-45\% increase in the supported traffic in their cases of study. The authors of MaskRSA also contributed to open source by releasing their simulation framework, RSA-RL.
    \item \textbf{PtrNet-RSA} \cite{cheng_ptrnet-rsa_2024} is a 2024 paper that presents innovation in both the problem setting and the function approximator. A pointer-net \cite{vinyals_pointer_2015} is used to select the constituent nodes of the target path, thereby removing the restriction of selecting from the pre-calculated k-shortest paths, and utilizes masking to allow selection from all available spectral slots. Additionally, the paper considers joint optimization of the mean path SNR and the network blocking probability through its reward function. It demonstrates superior performance to KSP-FF and their implementation of MaskRSA on both metrics. Arguably, PtrNet-RSA represents the apotheosis of current RL solutions for DRA problems, by combining the innovations from the other selected papers and considering a more complete problem context with physical layer model.
\end{enumerate}

DeepRMSA, Reward-RMSA, and GCN-RMSA use the same original DeepRMSA codebase as the basis for their experiments. Consequently, they all retain an idiosyncratic feature of that implementation, service holding time truncation, discussed in section \ref{sec:holding_time}. Another common characteristic is they use consider directed graphs with dual fiber links i.e. each link comprises two fibers, one for each direction of propagation. This doubles the maximum potential capacity of the network compared to single-fiber links. MaskRSA and PtrNet-RSA model single-fiber links, which makes the problem less challenging for RL due to less sparse reward signals (more frequent blocking) but also less similar to real-world optical networks. PtrNet-RSA does not consider distance-dependent modulation format.


\begin{figure}
  \includegraphics[width=0.5\textwidth]{IMAGES/networks_plots_short.png}
  \caption{Network topologies used in the case studies from influential papers: DeepRMSA, Reward-RMSA, GCN-RMSA, MaskRSA, PtrNetRSA \cite{chen_deeprmsa_2019} \cite{tang_heuristic_2022} \cite{xu_deep_2022} \cite{shimoda_mask_2021} \cite{cheng_ptrnet-rsa_2024}. The COST239 topology shown is from DeepRMSA, the USNET is from PtrNet-RSA.}
  \label{fig:network_plots}.
\end{figure}

Figure \ref{fig:network_plots} shows the topologies used in the selected publications. %Some characteristic features of the topologies are summarised in table \ref{tab:topology_features}.  
We note that the USNET topology differs between GCN-RMSA \cite{xu_deep_2022} and PtrNet-RSA \cite{cheng_ptrnet-rsa_2024}. We show the PtrNet version here with longer, more realistic link lengths. PtrNet-RSA also uses a unique variant of the COST239 topology. We make all topology data available \cite{micdoh_xlron_2024}






\subsection{Network traffic warmup}
\label{sec:warmup}

Network traffic warm-up is an important detail in RL solutions for RMSA that affects blocking probability statistics. During warm-up, traffic requests populate the network topology using either an RL policy or heuristic before training or evaluation begins. This pre-population serves two key purposes:

First, it helps prevent primacy bias \cite{nikishin_primacy_2022}, where models overfit to data seen early in training. When starting with an empty network, initial traffic requests are trivially allocated due to abundant resources, providing no useful optimization signal. Training on a congested network with both successful and failed assignments gives more meaningful training data from the start.

Second, warm-up helps the network reach a steady operating state more quickly. Without warm-up, episodes would need to be longer to achieve representative network conditions.

While most papers do not explicitly discuss warm-up, both the DeepRMSA codebase and RSA-RL framework from MaskRSA implement it. In section \ref{sec:repro}, we use this technique to match published results, adopting their 3000-request warm-up period. However, we also investigate how varying the warm-up length affects performance. We find that mean SBP stabilizes to steady state after a number of requests that depends on the traffic load. This suggests training and evaluation should only begin once steady state is reached. We therefore analyze the minimum required warm-up period for different traffic levels.

\subsubsection{Experiment setup}

We simulate a network that accepts all service requests (no blocking) to determine the number of requests needed to reach a steady state traffic load. Specifically, we define "steady state" as the point at which the number of active requests equals a target traffic load. Connection requests arrive according to an inverse exponential distribution with mean rate $\lambda$, and have holding times drawn from another inverse exponential distribution with mean $\tau$. The target traffic load is reached when $\lambda \tau$ connections are active in the network.

For each traffic load from 50 to 1000 Erlangs in steps of 50, we conduct 10,000 simulation trials. In each trial, we record how many requests must be generated before reaching steady state. We then aggregate these counts across trials to create box and whisker plots showing the distribution. From our initial experiments, we observe that the ratio of mean holding time to mean arrival rate does not affect the number of requests needed to reach steady state for a given traffic load. Therefore, we fix the mean holding time at 10 time units for all experiments.


\subsubsection{Results and discussion}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{IMAGES/steady_state_boxplots.png}
    \caption{No. of simulated requests necessary to reach target network traffic level for a non-blocking network.}
    \label{fig:traffic_warmup}
\end{figure}

Figure \ref{fig:traffic_warmup} displays results as box-and-whisker plots showing how many requests are needed to reach steady state for each traffic load. The whiskers extend to the most extreme data points (within 1.5 times the interquartile range). By fitting a line to the maximum values (tops of the whiskers), we can determine the requests needed to reach steady state with high probability. The fitted line indicates that approximately 7 times the target traffic load in requests are required to reach steady state. Based on this finding, the 3000-request warm-up period used by DeepRMSA and that we adopt in section \ref{sec:repro} is sufficient for most of our test scenarios.










\subsection{Holding time truncation}
\label{sec:holding_time}

In order to reproduce published results, its necessary to recreate every aspect of the traffic model. One feature of the traffic model in DeepRMSA and successor works is that the randomly sampled holding time is resampled if the resulting value is more than twice the mean of the inverse exponential PDF. We refer to this detail as holding time truncation. 


\subsubsection{Experiment setup}
To understand the effect of truncation on the traffic statistics, we define an inverse exponential PDF with unit mean. We take $10^{6}$ samples from the PDF, both with and without truncation, and calcualte the mean of the resulting samples in both cases.

\subsubsection{Results and discussion}
Figure \ref{fig:truncation} compares histograms of service holding times with and without truncation. The truncated case shows a sharp cutoff at twice the mean holding time, while the untruncated case follows the full exponential distribution. The vertical lines indicate the mean holding time for each case, revealing that truncation reduces the mean by approximately 31\%. This means that papers implementing holding time truncation (including DeepRMSA, Reward-RMSA, and GCN-RMSA) effectively evaluated their solutions at traffic loads 31\% lower than reported. While this implementation detail exists in the open source DeepRMSA codebase that these works built upon, it was not explicitly documented in the published papers themselves. This finding highlights the challenges in making fair comparisons when papers use non-standard implementations of the problem settings.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{IMAGES/truncation.png}
    \caption{Histogram of holding time for untruncated Poisson distribution with mean of 1. The untruncated distribution resamples the holding time when the sampled value exceeds 2*mean. This reduces the mean holding time by 31\% from the full Poisson distribution.}
    \label{fig:truncation}
\end{figure}









\subsection{Reproduction of published results}
\label{sec:repro}

Our analysis of the best performing heuristics and the implementation details of previous work (network warm-up and holding time truncation) enable us to perform a comprehensive benchmarking of the published results from the five selected influential papers. The aim of this comparison is to determine if any of the selected works have managed to exceed simple heuristic algorithms in performance on their cases of study. In order to do so, we recreate their simulations exactly and apply the KSP-FF heuristic algorithm with K=50 and paths ordered by number of hops in each case, based on our experiments from section \ref{sec:heuristic_comparison}.


\subsubsection{Experiment setup}


We recreate their cases of study in our own simulation framework \cite{doherty_xlron_2024} for fast, accurate, and reproducible results. We match the topologies (NSFNET, COST239, JPN48, USNET), mean service arrival rates, mean service holding times, data-rate request distributions, and traffic matrices. We analyzed the open source DeepRMSA codebase to identify holding time truncation and a network warmup period of 3000 steps. We corresponded with the authors of MaskRSA and PtrNet-RSA to find details of their simulations based on RSA-RL and identify the exact physical topologies used. We use the same measurement methodology as described in the respective papers to reproduce results, which is 3000 request warmup period followed by 10,000 requests. The SBP is calculated at the end of the episode. We perform 10 trials and calculate the mean and standard deviation across trials.

We extract published results from the publications, using textual values where available otherwise reading from charts. All published results report only a single data point for each traffic value, without any uncertainties. We check that our results for KSP-FF with K=5 match the published results within two standard deviations to ensure faithful reproduction. 



\subsubsection{Results and discussion}


\begin{figure*}
  \includegraphics[width=\textwidth]{IMAGES/review_summary_plots_2.png}
  \caption{Mean service blocking probability against traffic load. Each column is a publication and each subplot is for a topology. Error bars and shaded regions show standard deviations. Data for $RL$ and 5-SP-FF$_{published}$ are extracted from the publications. Close agreement between 5-SP-FF$_{published}$ and  5-SP-FF$_{ours}$ show that we accurately reproduce each case of study. \mbox{50-SP-FF$_{hops}$} exceeds or  matches the $RL$ performance for each case.}
  \label{fig:repro}
\end{figure*}

Figure \ref{fig:repro} shows our reproduction of results from the selected papers. Each subplot compares service blocking probability (SBP) against traffic load in Erlangs. The plots are organized by paper (columns) and topology (rows). PtrNet-RSA has two columns reflecting its two test cases: networks with 40 FSU per link handling 1 FSU requests, and networks with 80 FSU per link handling 1-4 FSU requests.

Each plot contains 5 datasets:
\begin{itemize}
\item[] \textbf{RL}: Published results for the reinforcement learning approach
\item[] \textbf{5-SP-FF$_{published}$}: Published results for 5-SP-FF with paths ordered by length
\item[] \textbf{5-SP-FF$_{ours}$}: Our reproduction of 5-SP-FF with paths ordered by length
\item[] \textbf{5-SP-FF$_{hops}$}: Our implementation of KSP-FF (K=5) with paths ordered by number of hops
\item[] \textbf{50-SP-FF$_{hops}$}: Our implementation of KSP-FF (K=50) with paths ordered by number of hops
\end{itemize}

Points show mean values from our simulations, with shaded areas indicating standard deviation and lines interpolating between points. DeepRMSA provides data for only one traffic load per topology.

We validate our simulation framework by comparing 5-SP-FF$_{published}$ to 5-SP-FF$_{ours}$. The excellent agreement across all cases confirms that our framework accurately reproduces the published scenarios. We do not attempt to reproduce the RL results directly, as this would require exact replication of all training details or access to the original trained models, neither of which are available. Instead, we extract the RL results from the papers and use the matching KSP-FF results to verify our simulations.

Our results show that KSP-FF$_{hops}$ with either K=5 or K=50 exceeds the published RL performance in most cases. Using K=50 matches or exceeds RL performance in all but one case. While our earlier experiments showed FF-KSP performs better than KSP-FF for JPN48, we only plot KSP-FF results as they already surpass the RL performance. For MaskRSA JPN48, FF-KSP with K=50 achieves zero blocking across all tested traffic loads.

The single exception where RL outperforms 50-SP-FF$_{hops}$ is PtrNet-RSA-80 USNET. Three factors may explain this:
\begin{enumerate}
    \item The RL results fall within 1-2 standard deviations of our heuristic mean. Without multiple trials from PtrNet-RSA, we cannot make a definitive comparison. Their favorable 5-SP-FF results suggest they may have used an advantageous random seed.
    \item PtrNet-RSA uses fixed-width requests without distance-dependent modulation, potentially allowing RL to exploit this simpler scenario.
    \item The pointer-net architecture can consider any possible path, unlike K-shortest path approaches. This broader search space likely enables better performance, similar to how increasing K improves KSP-FF.
\end{enumerate}

All data shown in figure \ref{fig:repro} is provided in tabular form in Appendix A.

% PtrNet also seeks to maximise the average GSNR of the active lightpaths, however this is closely linked to throughput.














































% \subsubsection*{Cut-Sets Capacity Bound Estimation}

% \begin{algorithm}
% \caption{Cut-Sets Capacity Bound}
% \begin{algorithmic}[1]
% \Require Network topology $G$, Traffic matrix $T$, Number of frequency slots per link $F$
% \Ensure Blocking probability $P_b$

% \State $N \gets \textsc{InitializeNetwork}(G, F)$ \Comment{Initialize network with empty spectrum slots}
% \State $C_{cong} \gets \textsc{IdentifyCutSets}(G, T, M)$ \Comment{Find congested cut-sets}
% \State $L_{map} \gets \textsc{MapLinksToCutSets}(G, C_{cong})$ \Comment{Map network links to cut-sets}
% \State $\textit{blocked} \gets 0$
% \State $\textit{total} \gets 0$

% \While{simulation not complete}
%     \For{each active request $r$ that expired}
%         \For{each link $l \in r.\textit{path}$}
%             \State \textsc{ReleaseSpectrum}($N[l]$, $r.\textit{slots}$)
%         \EndFor
%     \EndFor
    
%     \For{each new request $r(s,d)$}
%         \State $\textit{total} \gets \textit{total} + 1$
%         \State $m \gets \textsc{GetHighestModulation}(s, d)$
%         \State $req\_slots \gets \textsc{CalculateRequiredSlots}(r, m)$
        
%         \State $C_r \gets \{c \in C_{cong} | \textsc{Separates}(c, s, d)\}$
%         \State $available \gets \texttt{true}$
%         \State $candidate\_links \gets \emptyset$
        
%         \For{each cut-set $c \in C_r$}
%             \State $links \gets L_{map}[c]$ \Comment{Get network links in this cut-set}
%             \State $L_c \gets \{l \in links | \textsc{FreeSlots}(N[l], req\_slots)\}$
%             \If{$L_c = \emptyset$}
%                 \State $available \gets \texttt{false}$
%                 \State \textbf{break}
%             \EndIf
%             \State $candidate\_links[c] \gets L_c$
%         \EndFor
        
%         \If{$available$}
%             \State $sel\_links \gets \textsc{OnePerCutset}(candidate\_links)$
%             \State $sel\_slots \gets \textsc{GetSlots}(N, sel\_links, req\_slots)$
%             \If{$sel\_slots \neq \emptyset$}
%                 \For{each link $l \in sel\_links$}
%                     \State \textsc{AssignSlots}($N[l]$, $sel\_slots$, $req\_slots$)
%                 \EndFor
%                 \State $r.\textit{path} \gets sel\_links$
%                 \State $r.\textit{slots} \gets sel\_slots$
%             \Else
%                 \State $\textit{blocked} \gets \textit{blocked} + 1$
%             \EndIf
%         \Else
%             \State $\textit{blocked} \gets \textit{blocked} + 1$
%         \EndIf
%     \EndFor
% \EndWhile

% \State \Return $\textit{blocked}/\textit{total}$

% \end{algorithmic}
% \end{algorithm}

% ```

% The cut-set capacity bound algorithm utilizes seven key subroutines:

% \begin{itemize}
%     \item \textsc{InitializeNetwork}($G$, $F$) creates an empty network state with $F$ frequency slots available on each link in topology $G$.
    
%     \item \textsc{IdentifyCutSets}($G$, $T$, $M$) determines the most congested cut-sets by analyzing the ratio of expected traffic flow to available capacity across all possible network bisections, weighted by achievable modulation formats.
    
%     \item \textsc{MapLinksToCutSets}($G$, $C_{cong}$) creates a mapping from each congested cut-set to its constituent network links, ensuring that allocated resources on each cut set map to physical links.
    
%     \item \textsc{FreeSlots}($N[l]$, $req\_slots$) determines if link $l$ has sufficient contiguous free spectrum slots to accommodate the request.
    
%     \item \textsc{OnePerCutset}($candidate\_links$) selects exactly one link from each cut-set's candidate links such that the selected links can potentially support a common spectrum assignment. The selected link in each cutset is determined by the constituent links of the shortest available path.
    
%     \item \textsc{GetSlots}($N$, $sel\_links$, $req\_slots$) identifies a common set of contiguous spectrum slots available across all selected links using a first-fit policy.
    
%     \item \textsc{AssignSlots}($N[l]$, $sel\_slots$, $req\_slots$) allocates the selected spectrum slots on link $l$, maintaining the network state.
% \end{itemize}


==> archive/definition_of_terms.tex <==
\subsection*{Definition of terms}

We define the following terms used in this paper for the purposes of disambiguation:

\textbf{Path} - A series of network fibre links that comprise a route from source to destination nodes.

\textbf{Lightpath} - The path and specified bandwidth slice that constitute a connection from source to destination, and which obeys the spectrum continuity and contiguity constraints.

\textbf{Connection request} - Network data traffic comprises a series of connection requests; tuples of source node, destination node, and requested data rate. 

\textbf{Static traffic} - All connection requests are known a priori, can be allocated in any order, and do not expire.

\textbf{Dynamic traffic} - Future connection requests are unknown, are allocated sequentially, and expire.

\textbf{Fixed grid} - Available spectrum is partitioned in spectral slots of width 50 or 100 GHz.

\textbf{Flex-grid} - Available spectrum is partitioned into spectral slots of width 6.25GHz or greater, up to 37.5GHz.

\textbf{Flex-rate} - Available spectrum is fixed grid but each lightpath can support multiple connection requests until the available bandwidth of a lightpath is fully utilised, by adjusting data rate of transceiver.

\textbf{RWA} - The routing and wavelength allocation problem. The task is to assign lightpaths to connection requests on a fixed grid network, in order to minimise an objective or set of objectives e.g. no. of blocked connections, latency, no. of transceivers.

\textbf{RSA} - The routing and spectrum allocation problem. Identical to RWA but on a flex-grid substrate network.

\textbf{RMSA} - The routing, modulation and spectrum assignment problem. Identical to RSA but with the added constraint of SNR-dependent modulation format, whereby the bandwidth required to support a particular data rate on a lightpath depends on the available SNR, often assumed to be entirely distance-dependent. 

\textbf{DRA problems} - The umbrella term for dynamic resource allocation problems i.e. RWA, RSA, RMSA problems and variants. For the purposes of this review, this definition refers to problems that require routing of unicast traffic and do not consider node resources. This excludes problems such as network function virtualisation (NFV), virtual optical network embedding (VONE) and distributed sub-tree scheduling \cite{li_tabdeep_2024}. We exclude static traffic, for which exact solution methods are applicable.

==> archive/lit_edited.tex <==
x\subsection{Development of RL for DRA in optical networks}
\label{sec:survey-development}

In this section, we provide a survey of the progress in RL for DRA problems in optical networks. Our dataset of 96 collected papers (Figure \ref{fig:lit_barchart}) is useful to reveal trends in the research directions but we do not aim to discuss each paper in detail. Instead, we provide a narrative of the field's development, highlighting key papers and innovations. We choose to focus mainly on RWA/RSA/RMSA papers, to facilitate comparisons between works and construct a timeline of innovation.

We exclude many of the works gathered in our search from inclusion in this review, because we evaluate their contribution to the field as insignificant. In many cases, any claimed performance improvement is trivial due to comparison against only weak benchmarks, such as shortest path routing. %As we show in section \ref{sec:heuristic_comparison}, 




\subsubsection{Early works}
The first application of RL to network routing (in a packet switched network) was in 1993 \cite{boyan_packet_1993}, when Q-learning was used to continuously update a routing table for a 6x6 network. The optical networks community later picked up the technique in 2003 when Garcia et al investigated RL for multicast in WDM networks \cite{garcia_multicast_2003}. We note that multiple works then considered routing in Optical Burst Switched networks due to the research interest in that emerging networking paradigm at the time \cite{kiran_reinforcement_2006,belbekkouche_reinforcement_2008}. Koyanagi also \cite{koyanagi_reinforcement_2009} employed Q-learning for the task of service differentiation and noted the algorithm's sensitivity to hyperparameter selection. 

A significant milestone was achieved by the work of Pointurier and Heidari \cite{pointurier_reinforcement_2007}, which used the simple RL algorithm to update a routing table for a WDM network while accounting for quality of transmission (QoT) constraints, showing lower blocking probability than Shortest Path (SP) routing. This paper was the first to consider dynamic network traffic and to demonstrate improvement over a widely used heuristic, although it neglected to consider multiple candidate paths as KSP-FF. 

A decade later in 2017, Reyes amd Bauschert \cite{reyes_adaptive_2017} were the first to consider RL for dynamic traffic in flex-grid networks, again using a tabular approach. The modern era of RL, using deep neural networks as function approximators, was established by 2013 with the use of RL for Atari videogames (later published in Nature \cite{mnih_human-level_2015}). These more advanced techniques then began to be applied in optical networks in 2018, when the original DeepRMSA paper was presented at conference \cite{chen_deep-rmsa_2018}. We deascribe DeepRMSA in section \ref{sec:} This seminal paper spurred a series of incremental advances from 2019 onwards.




\subsection{Simulation and training libraries}
\label{sec:simulation_libraries}
Following DeepRMSA, there was a rise in publications on RL for DRA problems, as seen in Figure \ref{fig:lit_barchart}. This research was enabled by optical network simulation tools designed for RL training. Several open source toolkits have been introduced to aid researchers and improve productivity, but none has proved sufficiently popular for it to become the de facto standard. Optical-rl-gym \cite{natalino_optical_2020} was the first paper to attempt to introduce a new standard library for this task. This was followed by an extension to multi-band environments \cite{morales_multi-band_2021} and in 2024 was further extended to include a more sophisticated physical layer model for lightpath SNR calculations, renamed as the Optical Networking Gym \cite{natalino_optical_2024}. Meanwhile, the authors of MaskRSA open-sourced their simulation framework (RSA-RL) and DeepRMSA's codebase continued to be widely used. SDONSim \cite{mccann_sdonsim_2024} and DREAM-ON-GYM \cite{jara_dream-gym_2024} are other recent additions to the landscape of available simulation frameworks that further fragment the available options. In this work we use XLRON \cite{doherty_xlron_2023} the framework introduced at Optical Fibre Communications (OFC) 2024 that we continue to develop. We outline its benefits and justify its use in section \ref{sec:empirical_analysis}.



\subsubsection{DeepRMSA and feature engineering}
\label{sec:survey-deeprmsa}

DeepRMSA \cite{chen_deeprmsa_2019} is the most influential paper on RL for DRA, as measured by citations. It's notable as the first paper to achieve lower blocking probability than KSP-FF, through its use of a multi-layer perceptron (MLP) neural network as a function approximator for the learned policy, and its feature engineering of the observation space to enable more efficient learning. %This success sparked a series of successor works. We define successor works as papers that (i) use DeepRMSA as a benchmark, and/or (ii) show evidence of using the DeepRMSA codebase.
The impact of DeepRMSA is enhanced by its open source codebase, which has been used extensively by other researchers \cite{tang_heuristic_2022,xu_deep_2022,quang_magc-rsa_2022}.

Similar to DeepRMSA, in a contemporaneous work Su\'arez-Varela et al. \cite{suarez-varela_routing_2019} explored different state representations to aid learning. The paper is notable for its in-depth exploration of the effect of hyperparameters and network topology on the RL performance, and its thoughtful design of the observation space. It was less impactful than DeepRMSA perhaps because it benchmarked against shortest path routing only. A similar approach to feature engineering to aid the learning process was carried out by Tanaka and Shimoda \cite{tanaka_pre-_2023} in 2023, where they encode path information into the matrix of FSUs and links and use it to train an RL policy that is superior to KSP-FF in terms of blocking probability. Cruzado et al. also use path-based feature engineering in their work from 2022 \cite{cruzado_reinforcement-learning-based_2022}, but in general such manual feature engineering has been rejected in favour of end-to-end learning, particularly with graph neural networks (GNNs).


\subsubsection{Graph neural networks}
\label{sec:gnn_rl}

GNNs are well-suited to optical networking problems due to their inductive bias for graph-structured data \cite{xu_how_2018}. 


Then Quang et al. introduced MAGC-RSA \cite{quang_magc-rsa_2022}, which utilizes invalid action masking like MaskRSA, the shaped reward from Reward-RMSA \cite{tang_heuristic_2022}, and a graph convolutional neural network like GCN-RMSA \cite{xu_deep_2022}. They claim it is multi-agent with a separate agent at each node, but actually they use a standard GNN with attention, and they claim it is better than KSP-FF and (their implementation of) DeepRMSA. However, they do not consider distance-dependent modulation format.

 \cite{suarez-varela_graph_2023} \cite{li_gnn-based_2022}  Another GNN-RNN based paper here \cite{xiong_graph_2024}
 
 \cite{almasan_deep_2022} examines RSA as a use case for GNN's coupled with RL, with a particular focus on GNNs ability to generalise to topologies unseen during training. They find that the GNN-RL approach does not perform as well as a theoretical fluid model for network routing on unseen topologies, so generalization of RL-trained network routing policies remains an open problem.
 
 % MORE ADVANCED FUNCTION APPROXIMATORS
 
 More exotic deep learning architectures have also been employed for DRA problems. Optic-GAI \cite{li_opticgai_2024} uses a diffusion model, a generative model based on an iterative de-noising process and most often applied to image synthesis \cite{ho_denoising_2020}, as represent the RWA policy. The authors claim that this model is superior to KSP-FF for RWA but do not specify how many paths they consider.
 
 \cite{cheng_ptrnet-rsa_2024}
 

 


\subsubsection{Other techniques}
\label{sec:other_tehcniques}
% Talk about invalid action masking and reward shaping


Then Shimoda et al. make a significant contribution in two papers that introduced the concept originally referred to as assignable boundary slot mask \cite{shimoda_deep_2021} and then invalid action masking in the work MaskRSA \cite{shimoda_mask_2021}. The concept of invalid action masking was already well-known in the field of RL following its use in the AlphaStar paper from Google Deepmind \cite{vinyals_grandmaster_2019} and subsequent empirical investigations \cite{huang_closer_2020} but MaskRSA was the first paper to introduce it to optical networking, and contemporaneously with works on data centre networks \cite{shabka_resource_2021}.





\subsection{Emerging research trends}
\label{sec:survey-emerging_trends}

\cite{hernandez-chulde_experimental_2023} Latency awareness
\cite{nallaperuma_interpreting_2023} multi-objective RL


Another significant paper from 2022 from Nevin et al. \cite{nevin_techniques_2022}  is on techniques for the application of RL to RWA; specifically 1) invalid action masking and 2) scaling the network capacity to reduce the episode length. It poses a novel problem setting that seeks to closely replicate the resource allocation problem in most production networks of incremental traffic on a fixed-grid (100GHz per wavelength) with re-use of existing lightpaths with spare capacity to accommodate additional traffic (so-called "RWA with lightpath re-use" or RWA-LR). The merits of the work are multiple; it presents a novel but realistic problem setting with a physical layer model that calculates lightpath capacities based on a simple GN model and Nyquist assumptions, it elaborates on the invalid action masking technique initially introduced to the field by MaskRSA \cite{shimoda_mask_2021}, and it articulates the fundamental difficulty of long episode lengths (i.e. sparse rewards) in the application of RL to this problem. It does, however, suffer from the common problem of benchmarking against the weaker KSP-FF heuristic with paths ordered by length. %We have recreated the RWA-LR problem setting in XLRON and applied KSP-FF with both path orderings to confirm our recreation accords with Nevin et al.. Our initial experiments confirm that ordering by number of hops allows greater throughput.


Xu et al. investigate a hierarchical framework for multi-domain networks \cite{xu_hierarchical_2023}

Multi-objective optimization of network condition is an emerging trend \cite{cheng_ptrnet-rsa_2024,xie_physical_2024,teng_deep-reinforcement-learning-based_2024}

Other problems could bear more fruit e.g. channel power optimization \cite{arpanaei_launch_2023,xiao_channel_2024}.

==> archive/network_blocking_bound_review.tex <==
\subsection{Network capacity bound estimation}
\label{sec:survey-capacity_bounds}

We conclude our review with a discussion of the network capacity bound estimation methods that have been used in the literature, in anticipation of introducing our technique in section \ref{sec:bounds}.

Recent work has applied the max-flow min-cut theorem from graph theory to estimate upper bounds on optical network capacity. This theorem states that the maximum flow possible between two nodes in a network equals the minimum cut capacity separating those nodes \cite{ford_maximal_1956}. A graph cut is a partition of the graph's nodes into two disjoint sets, the cut-set is the set of links crossing the cut, and the cut capacity is the sum of the capacities of the cut-set.

Hayashi et al. first adapted the concept of cut-sets analysis, originally developed for packet-switched networks, and applied it to optical networks in their work on bit-rate variable virtual direct links \cite{hayashi_efficient_2022,hayashi_cost-effective_2023}. The method provides an upper bound on network capacity by relaxing the spectrum continuity constraint - it only considers spectrum allocation on the links in the minimum cut-set rather than ensuring continuous spectrum along full paths. This relaxation means the bound is not necessarily achievable in practice but provides a useful estimated upper bound limit. 

Cruzado et al. then extended this approach, first applying it to fixed-grid WDM networks to estimate capacity bounds for RWA \cite{cruzado_effective_2023}.  Most recently, they adapted the method for flex-grid elastic optical networks with distance-adaptive modulation formats \cite{cruzado_capacity-bound_2024}, providing theoretical bounds that account for path-dependent spectral efficiency.

The cut-sets method provides a useful upper bound estimate but is imperfect due to its reliance on a heuristic method (e.g. first-fit) to allocate the spectrum on the cut-set links. Sub-optimal allocation can cause spectrum fragmentation, thereby reducing the estimate and its reliability as a true upper bound. We propose a novel defragmentation-based method to estimate network capacity bounds in section \ref{sec:bounds}, which relaxes the constraint on reconfiguration instead of spectrum continuity.


==> archive/path_ordering_analysis.tex <==
\subsection{Path ordering}
\label{sec:path_ordering}

We find that ordering the K-shortest pre-calculated paths by number of hops gives lower blocking probability than ordering by distance in km. We refer to these two path orderings as \#hops and \#km, respectively. In this section, we address two potential criticisms of using \#hops ordering:
1) Ordering by \#hops results in unacceptable increases in path length in km.
2) Benchmarking RL solutions that use \#km ordering against heuristics with \#hops ordering is unfair, as the RL method did not have access to the same paths.

\subsubsection{Experiment setup}

We run two separate experiments to address the criticisms. We repeat these experiments for each of our test topologies.

First, we calculate the K-shortest paths for K=5 and K=50 for \#hops and \#km. We calculate the mean and standard deviation of the path lengths in hops and km for each of these cases.

Second, we run incremental traffic until the first blocking event and allocate traffic with KSP-FF for K=5 and K=50 for \#hops and \#km. We choose incremental traffic with first blocking as it allows a fairer comparison across topologies than dynamic traffic with arbitrary traffic loads. We record the paths selected in each case. We aim to investigate how the available paths differ between the two orderings, expressed as the percentage of paths that are unique to the ordering. 

We compare the differences in paths between \#hops and \#km for each case and plot: 1) \textbf{Available} shows what percentage of all pre-calculated paths between node pairs are unique when comparing the two orderings. 2) \textbf{Utilized} shows what percentage of paths that are selected by the heuristics to carry active connections are unique between the two orderings. We calculate the mean and upper and lower inter-quartile range values from 10 trials. We use the IQR to avoid unphysical negative values.

\subsubsection{Results and discussion}

Figure \ref{fig:length_hops_dotplot} compares the path lengths in both hops (y-axis) and km (x-axis) from Experiment 1. The figure shows that the difference in mean path length in km between \#hops and \#km ordering is notable but not prohibitive, with mean increases of approximately 20\% or less in length. The total throughput is still higher (SBP is lower), therefore this path length increase is not consequential. A problem specification that takes into account all physical layer effects and losses could make \#km ordering more favourable, e.g. by reducing mean latency, but for an optimization objective of network throughput, \#hops ordering is superior.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{IMAGES/length_hops_dotplot_50alt.png}
    \caption{The mean and standard deviation for path length in km and hops for each topology, KSP-FF ordered by length in km or hops, for K=5 and K=50. Increasing K from 5 to 50 has little effect on mean path length in km. Ordering by hops instead of distance increases the mean path length by a greater amount, dependent on the topology.}
    \label{fig:length_hops_dotplot}
\end{figure}

Figure \ref{fig:unique_paths_barchart} shows that \#hops and \#km orderings have 20-35\% dissimilar paths for K=5 and K=50 for NSFNET, COST239, and USNET. JPN48 is an outlier with over 50\% differences in the available paths for \#hops and \#km for both K=5 and K=50. However, examination of the utilized paths shows that allowing sufficient path diversity (K=50) means there is less than 1\% difference in utilized paths between \#hops and \#km for NSFNET, COST239, and USNET. This shows that, when training RL policies for DRA problems, it is important to have sufficient path options for the RL to equal the performance of a K-shortest path heuristic. However, for JPN48, significant differences (>20\%) between paths for \#hops and \#km are still evident even when only considering utilized paths, therefore it is is ultimately important to evaluate path orderings and select the optimal one to give RL the greatest chance at success.


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{IMAGES/unique_paths_barchart_50alt.png}
    \caption{The percentage of the K pre-calculated paths that are unique to the path ordering (path length in km or hops) for each topology for K=5 and K=20. "Available" shows the percentage of paths available to choose from. "Utilised" shows the mean percentage of paths that are unique to the path ordering and utilized by the KSP-FF or KSP-FF$_{hops}$ heuristics in an incremental loading scenario. Error bars show interquartile range.}
    \label{fig:unique_paths_barchart}
\end{figure}


==> archive/reinforcement_learning_review.tex <==
\subsection{Reinforcement learning}
\label{sec:background_rl}

RL is a framework for learning to optimize sequential decision making under uncertainty. It emerged from Bellman's foundational work on optimal control theory in the 1950s, specifically dynamic programming and Markov Decision Processes (MDP) \cite{bellman_theory_1954,bellman_markovian_1957}. MDPs model decision making processes as an agent, that takes actions, and the environment, with which it interacts. The environment transitions to a new state in response to an action, with a feedback signal (reward) provided to the agent. The method by which the agent decides on actions, in response to observation of the environment state, is termed the policy. RL algorithms describe how to iteratively improve the policy to maximize reward in the long term or within a fixed number of decision steps (an episode). RL is distinct from other machine learning paradigms, supervised and unsupervised learning, by removing the train-test dichotomy and instead learning from an interactive environment that produces data (observations and rewards). The policy is improved on the basis of this data, which in turn affects the data collection process, and presents a non-stationary optimization objective. A key distinction in RL algorithms is whether they learn from data collected using the current policy being optimized (on-policy learning) or from data collected using any policy, including previous or exploratory policies (off-policy learning) - the latter offering more data efficiency but potentially greater instability during training.

While dynamic programming is restricted to problems with completely known dynamics, reinforcement learning allows the foundational ideas of state-value estimation and policy iteration to be applied to problems with incomplete knowledge of the state transition dynamics, as in the case of dynamic networks with unknown future traffic. This broad applicability of reinforcement earning techniques was enabled by later developments in the 80s and 90s of Q-learning \cite{watkins_learning_1989}, temporal difference learning \cite{sutton_learning_1988}, and actor-critic algorithms. The modern era of reinforcement learning was brought in by ground-breaking works from researchers at what is now Google Deepmind in the domains of Atari videogames \cite{mnih_human-level_2015} and the boardgame Go \cite{silver_mastering_2016}. These works demonstrated the effectiveness of RL algorithms, specifically Q-learning, when combined with deep neural networks (DNN) as function approximators.

We do not provide details of reinforcement learning theory here and instead refer the reader to Sutton and Barto's authoritative textbook \cite{sutton_reinforcement_2018}. However, to aid the discussion of RL applied to DRA problems, we outline the taxonomy of the RL algorithms as follows:

\textbf{Model-free} RL algorithms learn optimal behavior through direct interaction with the environment, without explicitly modeling its dynamics. These algorithms can be further categorized into:
\begin{itemize}
\item \textbf{Action-value methods}, such as Q-learning and SARSA, which learn to estimate the value of taking specific actions in different states. These methods were the first to be developed in RL.
\item \textbf{Policy gradient methods}, which directly optimize the policy parameters to maximize expected rewards. These methods can be applied to continuous action spaces and can naturally handle stochastic policies. Policy gradient methods are enhanced by using an Actor-Critic architecture, including algorithms such as A2C, PPO, and off-policy variants like DDPG and SAC, which reduce variance in the policy gradient by using a learned value function (critic) to estimate the value of each state, rather than using the full Monte Carlo returns.

\end{itemize}
\textbf{Model-based} RL algorithms use an explicit model of the environment's dynamics alongside the policy. The model may be an available simulator, as in AlphaGo \cite{silver_mastering_2016} or can be learned, as in MuZero \cite{silver_general_2018}. The model is used to simulate experience for a search process (e.g. Monte Carlo Tree Search) over possible trajectories, enabling multi-step planning to maximize reward. This leads to considerably higher performance in complex tasks, at the cost of much higher computational complexity \cite{brown_superhuman_2019}.
In the context of optical networks, only model-free algorithms have been applied to DRA problems thus far in the research literature.


% \begin{equation}
%     \label{eq:bellman_optimality}
%     V^*(s) = \max_a \left( R(s,a) + \gamma \sum_{s'} P(s'|s,a) V^*(s') \right)
% \end{equation}
% Equation \ref{eq:bellman_optimality} is the Bellman optimality equation, a fundamental principle in RL that defines the optimal value function. It states that the optimal value of a state is equal to the expected return for the best action from that state. This equation forms the basis for many RL algorithms, including value iteration and Q-learning, and provides a mathematical framework for understanding how agents can make optimal decisions in sequential decision-making problems.

% \begin{equation}
%     \label{eq:bellman_optimality_q}
%     Q^*(s,a) = R(s,a) + \gamma \sum_{s'} P(s'|s,a) \max_{a'} Q^*(s',a')
% \end{equation}
% Equation \ref{eq:bellman_optimality_q}, the Q-function version of the Bellman optimality equation, defines the optimal action-value function in reinforcement learning. It represents the expected return of taking action a in state s and then following the optimal policy thereafter. This equation is crucial in Q-learning and other value-based methods, as it allows for optimal action selection without requiring a model of the environment. The Q-function directly incorporates the action into the value estimation, making it particularly useful for control problems.

==> archive/results_table_20.tex <==
%\onecolumn
%\centering
%\scriptsize

\newpage
\onecolumn
\appendix
\section{Appendix: Data from published work and our reproductions}
\label{appendix:A}
\nopagebreak
\setlength{\tabcolsep}{6pt}
\begin{longtable}[!htbp]{llll|lllll|l}


\caption{Comparison of service blocking probabilities for KSP-FF and RL solutions across various topologies and traffic loads.}\label{tab:blocking_probabilities} \\
\hline
\multirow{3}{*}{\textbf{Publication}} & \multirow{3}{*}{\textbf{Topology}} & \multirow{3}{*}{\textbf{N$_{slots}$}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Load \\ (Erlang)\end{tabular}}} & \multicolumn{5}{c|}{\textbf{Service blocking probability (\%)}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mean \\ improvement \\ over RL (\%)\end{tabular}}} \\
\cline{5-9}
 &  &  &  & \multicolumn{2}{c|}{Published} & \multicolumn{3}{c|}{Ours} &  \\
\cline{5-9}
 &  &  &  & RL & \multicolumn{1}{c|}{5-SP-FF} & 5-SP-FF & 5-SP-FF$_{hops}$ & 20-SP-FF$_{hops}$ &  \\
\hline
\endfirsthead

\multicolumn{10}{c}{Table \thetable{} -- continued from previous page} \\
\hline
\multirow{3}{*}{\textbf{Publication}} & \multirow{3}{*}{\textbf{Topology}} & \multirow{3}{*}{\textbf{N$_{slots}$}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Load \\ (Erlang)\end{tabular}}} & \multicolumn{5}{c|}{\textbf{Service blocking probability (\%)}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mean \\ improvement \\ over RL (\%)\end{tabular}}} \\
\cline{5-9}
 &  &  &  & \multicolumn{2}{c|}{Published} & \multicolumn{3}{c|}{Ours} &  \\
\cline{5-9}
 &  &  &  & RL & \multicolumn{1}{c|}{5-SP-FF} & 5-SP-FF & 5-SP-FF$_{hops}$ & 20-SP-FF$_{hops}$ & \\
\hline
\endhead

\hline
\multicolumn{10}{r}{Continued on next page} \\
\endfoot

\hline
\endlastfoot



% START FIX

%\textbf{Publication} & \textbf{Topology} & \textbf{N$_{slots}$} & \textbf{\begin{tabular}[c]{@{}l@{}}Load \\ (Erlang)\end{tabular}} & \multicolumn{5}{c|}{\textbf{Blocking probability  (\%)}}                                 & \textbf{\begin{tabular}[c]{@{}l@{}}Improvement \\ over RL (\%)\end{tabular}} & \textbf{} & \textbf{} & \textbf{} \\ \cline{5-9}
%                     &                   &                      &                                                                   & \multicolumn{2}{c|}{Published}      & \multicolumn{3}{c|}{Ours}                          &                                                                                         \\ \cline{5-9}
%                     &                   &                      &                                                                   & RL   & \multicolumn{1}{l|}{5-SP-FF} & 5-SP-FF     & 5-SP-FF$_{hops}$ & 20-SP-FF$_{hops}$ &                                                                                         \\ \cline{1-10}


% END FIX
                     
DeepRMSA             & NSFNET            & 100                  & 250                                                               & 4.00    & \multicolumn{1}{l|}{5.10}     & 5.13 ± 0.32 & 3.07 ± 0.20      &                   & 23                                                                                    \\
DeepRMSA             & COST239           & 100                  & 600                                                               & 5.75 & \multicolumn{1}{l|}{6.75}    & 6.69 ± 0.35  & 4.04 ± 0.33      &                   & 30                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 168                                                               & 0.35  & \multicolumn{1}{l|}{1.00}       & 1.11 ± 0.15  & 0.13 ± 0.06       &                   & 63                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 182                                                               & 0.70  & \multicolumn{1}{l|}{1.40}       & 1.59 ± 0.22  & 0.32 ± 0.10       &                   & 54                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 196                                                               & 1.20  & \multicolumn{1}{l|}{2.10}       & 2.19 ± 0.28  & 0.66 ± 0.22       &                   & 45                                                                                    \\
Reward-RMSA          & NSFNET            & 100                  & 210                                                               & 1.80  & \multicolumn{1}{l|}{2.70}       & 2.87 ± 0.29  & 1.14 ± 0.31       &                   & 37                                                                                    \\                                                      
GCN-RMSA             & NSFNET            & 100                  & 154                                                               & 0.51 & \multicolumn{1}{l|}{0.67}    & 0.78 ± 0.10 & 0.06 ± 0.05      &                   & 88                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 168                                                               & 0.66 & \multicolumn{1}{l|}{1.00}       & 1.11 ± 0.15 & 0.13 ± 0.06      &                   & 80                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 182                                                               & 0.98 & \multicolumn{1}{l|}{1.42}    & 1.59 ± 0.22 & 0.32 ± 0.10      &                   & 67                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 196                                                               & 1.50  & \multicolumn{1}{l|}{2.10}     & 2.19 ± 0.28 & 0.66 ± 0.22      &                   & 56                                                                                    \\
GCN-RMSA             & NSFNET            & 100                  & 210                                                               & 2.10  & \multicolumn{1}{l|}{2.76}    & 2.87 ± 0.29 & 1.14 ± 0.31      &                   & 46                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 368                                                               & 0.71 & \multicolumn{1}{l|}{0.78}    & 0.78 ± 0.21 & 0.09 ± 0.07      &                   & 87                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 391                                                               & 0.85 & \multicolumn{1}{l|}{1.30}     & 1.03 ± 0.24    & 0.14 ± 0.09      &                   & 84                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 414                                                               & 1.25 & \multicolumn{1}{l|}{1.70}     & 1.46 ± 0.27 & 0.26 ± 0.14      &                   & 79                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 437                                                               & 1.75 & \multicolumn{1}{l|}{2.30}     & 1.84 ± 0.34 & 0.49 ± 0.26      &                   & 72                                                                                    \\
GCN-RMSA             & COST239           & 100                  & 460                                                               & 2.10  & \multicolumn{1}{l|}{2.70}     & 2.39 ± 0.31 & 0.63 ± 0.19      &                   & 70                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 320                                                               & 0.65 & \multicolumn{1}{l|}{0.75}    & 1.02 ± 0.28 & 0.23 ± 0.13      &                   & 65                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 340                                                               & 0.83 & \multicolumn{1}{l|}{1.20}     & 1.27 ± 0.33 & 0.47 ± 0.20      &                   & 43                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 360                                                               & 1.05 & \multicolumn{1}{l|}{1.50}     & 1.67 ± 0.30 & 0.74 ± 0.10      &                   & 30                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 380                                                               & 1.60  & \multicolumn{1}{l|}{2.15}    & 2.25 ± 0.43 & 1.17 ± 0.20      &                   & 27                                                                                    \\
GCN-RMSA             & USNET             & 100                  & 400                                                               & 2.20  & \multicolumn{1}{l|}{2.70}     & 2.72 ± 0.42 & 1.62 ± 0.21      &                   & 26                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 80                                                                & 0.01 & \multicolumn{1}{l|}{0.26}    & 0.33 ± 0.04 & 0.00 ± 0.00            &                   & 100                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 90                                                                & 0.05 & \multicolumn{1}{l|}{0.60}     & 0.66 ± 0.09 & 0.01 ± 0.01           &                   & 80                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 100                                                               & 0.20  & \multicolumn{1}{l|}{0.90}     & 1.08 ± 0.10  & 0.08 ± 0.04            &                   & 60                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 110                                                               & 0.50  & \multicolumn{1}{l|}{1.80}     & 1.68 ± 0.10  & 0.25 ± 0.08            &                   & 50                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 120                                                               & 0.79 & \multicolumn{1}{l|}{2.47}    & 2.31 ± 0.18 & 0.62 ± 0.16      &                   & 22                                                                                    \\
MaskRSA              & NSFNET            & 80                   & 130                                                               & 1.80  & \multicolumn{1}{l|}{3.00}       & 3.22 ± 0.15 & 1.38 ± 0.21            &                   & 23                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 140                                                               & 3.00    & \multicolumn{1}{l|}{4.00}       & 4.09 ± 0.19 & 2.30 ± 0.21            &                   & 23                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 150                                                               & 4.30  & \multicolumn{1}{l|}{5.00}       & 5.11 ± 0.22 & 3.37 ± 0.31           &                   & 22                                                                                     \\
MaskRSA              & NSFNET            & 80                   & 160                                                               & 5.30  & \multicolumn{1}{l|}{6.00}       & 6.25 ± 0.25 & 4.59 ± 0.21            &                   & 13                                                                                     \\
MaskRSA              & JPN48             & 80                   & 120                                                               & 0.05 & \multicolumn{1}{l|}{1.60}     & 1.91 ± 0.21 & 0.32 ± 0.07      & 0.09 ± 0.04       & -80                                                                                     \\
MaskRSA              & JPN48             & 80                   & 130                                                               & 0.20  & \multicolumn{1}{l|}{2.50}     & 2.80 ± 0.33  & 0.62 ± 0.08      & 0.14 ± 0.03       & 30                                                                                      \\
MaskRSA              & JPN48             & 80                   & 140                                                               & 0.55 & \multicolumn{1}{l|}{3.50}     & 3.63 ± 0.33 & 1.00 ± 0.13         & 0.22 ± 0.04       & 60                                                                                      \\
MaskRSA              & JPN48             & 80                   & 150                                                               & 0.90  & \multicolumn{1}{l|}{4.50}     & 4.56 ± 0.31 & 1.46 ± 0.20       & 0.37 ± 0.10        & 59                                                                                    \\
MaskRSA              & JPN48             & 80                   & 160                                                               & 1.60  & \multicolumn{1}{l|}{5.00}       & 5.48 ± 0.41 & 1.96 ± 0.24      & 0.62 ± 0.09       & 61                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 180                                                               & 0.01 & \multicolumn{1}{l|}{0.80}     & 0.91 ± 0.28 & 0.00 ± 0.00            &                   & 100                                                                                     \\
PtrNet-RSA           & NSFNET            & 40                   & 190                                                               & 0.03 & \multicolumn{1}{l|}{1.25}    & 1.23 ± 0.28 & 0.00 ± 0.01         &                   & 100                                                                                     \\
PtrNet-RSA           & NSFNET            & 40                   & 200                                                               & 0.08 & \multicolumn{1}{l|}{1.50}     & 1.67 ± 0.31 & 0.02 ± 0.03      &                   & 75                                                                                      \\
PtrNet-RSA           & NSFNET            & 40                   & 210                                                               & 0.19 & \multicolumn{1}{l|}{1.90}     & 1.98 ± 0.34 & 0.07 ± 0.06      &                   & 63                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 220                                                               & 0.23 & \multicolumn{1}{l|}{2.50}     & 2.47 ± 0.43 & 0.20 ± 0.12       &                   & 13                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 230                                                               & 0.75 & \multicolumn{1}{l|}{2.90}     & 2.99 ± 0.48 & 0.41 ± 0.19      &                   & 45                                                                                    \\
PtrNet-RSA           & NSFNET            & 40                   & 240                                                               & 1.30  & \multicolumn{1}{l|}{3.50}     & 3.81 ± 0.71 & 0.80 ± 0.32       &                   & 38                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 340                                                               & 0.01 & \multicolumn{1}{l|}{2.50}     & 3.07 ± 0.37 & 0.02 ± 0.02      &                   & -100                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 360                                                               & 0.04 & \multicolumn{1}{l|}{3.25}    & 3.60 ± 0.43  & 0.03 ± 0.03      &                   & 25                                                                                      \\
PtrNet-RSA           & COST239           & 40                   & 380                                                               & 0.12 & \multicolumn{1}{l|}{3.80}     & 4.26 ± 0.51 & 0.07 ± 0.03      &                   & 42                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 400                                                               & 0.24 & \multicolumn{1}{l|}{4.60}     & 4.92 ± 0.52 & 0.16 ± 0.08      &                   & 33                                                                                    \\
PtrNet-RSA           & COST239           & 40                   & 420                                                               & 0.39 & \multicolumn{1}{l|}{5.50}     & 5.73 ± 0.71 & 0.37 ± 0.17      &                   & 5                                                                                   \\
PtrNet-RSA           & USNET             & 40                   & 210                                                               & 0.01 & \multicolumn{1}{l|}{0.85}    & 1.01 ± 0.16 & 0.14 ± 0.06      & 0.01 ± 0.02       & 0                                                                                       \\
PtrNet-RSA           & USNET             & 40                   & 220                                                               & 0.08 & \multicolumn{1}{l|}{1.40}     & 1.44 ± 0.22 & 0.27 ± 0.08      & 0.03 ± 0.04       & 63                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 230                                                               & 0.22 & \multicolumn{1}{l|}{1.85}    & 1.93 ± 0.29 & 0.47 ± 0.15      & 0.05 ± 0.05       & 77                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 240                                                               & 0.38 & \multicolumn{1}{l|}{2.20}     & 2.54 ± 0.35 & 0.79 ± 0.21      & 0.17 ± 0.14       & 55                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 250                                                               & 0.68 & \multicolumn{1}{l|}{3.10}     & 3.16 ± 0.43 & 1.18 ± 0.27      & 0.35 ± 0.20        & 49                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 260                                                               & 1.10  & \multicolumn{1}{l|}{3.60}     & 3.89 ± 0.49 & 1.73 ± 0.34      & 0.58 ± 0.30        & 47                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 270                                                               & 1.80  & \multicolumn{1}{l|}{4.40}     & 4.53 ± 0.42 & 2.42 ± 0.47      & 0.93 ± 0.41       & 48                                                                                    \\
PtrNet-RSA           & USNET             & 40                   & 280                                                               & 2.20  & \multicolumn{1}{l|}{4.90}     & 5.40 ± 0.46  & 3.12 ± 0.54      & 1.33 ± 0.46       & 40                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 200                                                               & 0.01 & \multicolumn{1}{l|}{0.60}     & 0.55 ± 0.17 & 0.00 ± 0.00            &                   & 100                                                                                     \\
PtrNet-RSA           & NSFNET            & 80                   & 210                                                               & 0.03 & \multicolumn{1}{l|}{0.80}     & 0.74 ± 0.15 & 0.00 ± 0.00            &                   & 100                                                                                     \\
PtrNet-RSA           & NSFNET            & 80                   & 220                                                               & 0.11 & \multicolumn{1}{l|}{1.20}     & 1.00 ± 0.23    & 0.01 ± 0.02      &                   & 91                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 230                                                               & 0.16 & \multicolumn{1}{l|}{1.40}     & 1.17 ± 0.23 & 0.03 ± 0.02      &                   & 81                                                                                    \\
PtrNet-RSA           & NSFNET            & 80                   & 240                                                               & 0.50  & \multicolumn{1}{l|}{1.90}     & 1.40 ± 0.28  & 0.06 ± 0.03      &                   & 88                                                                                      \\
PtrNet-RSA           & COST239           & 80                   & 420                                                               & 0.01 & \multicolumn{1}{l|}{2.50}     & 2.33 ± 0.40  & 0.07 ± 0.03      &                   & -600                                                                                    \\
PtrNet-RSA           & COST239           & 80                   & 440                                                               & 0.16 & \multicolumn{1}{l|}{3.00}       & 2.83 ± 0.38 & 0.11 ± 0.04      &                   & 31                                                                                    \\
PtrNet-RSA           & COST239           & 80                   & 460                                                               & 0.65 & \multicolumn{1}{l|}{3.50}     & 3.16 ± 0.51 & 0.19 ± 0.06      &                   & 71                                                                                    \\
PtrNet-RSA           & USNET             & 80                   & 260                                                               & 0.03 & \multicolumn{1}{l|}{1.00}       & 1.21 ± 0.22 & 0.47 ± 0.15      & 0.14 ± 0.12       & -367                                                                                 \\
PtrNet-RSA           & USNET             & 80                   & 270                                                               & 0.09 & \multicolumn{1}{l|}{1.20}     & 1.46 ± 0.23 & 0.62 ± 0.16      & 0.26 ± 0.14       & -189                                                                                 \\
PtrNet-RSA           & USNET             & 80                   & 280                                                               & 0.15 & \multicolumn{1}{l|}{1.40}     & 1.72 ± 0.29 & 0.80 ± 0.20        & 0.38 ± 0.22       & -153                                                                                 \\
PtrNet-RSA           & USNET             & 80                   & 290                                                               & 0.29 & \multicolumn{1}{l|}{1.70}     & 2.07 ± 0.26 & 1.12 ± 0.29      & 0.53 ± 0.25       & -83                                                                                  \\
PtrNet-RSA           & USNET             & 80                   & 300                                                               & 0.52 & \multicolumn{1}{l|}{2.20}     & 2.41 ± 0.33 & 1.36 ± 0.31      & 0.69 ± 0.25       & -33                                                                                  \\
PtrNet-RSA           & USNET             & 80                   & 310                                                               & 0.66 & \multicolumn{1}{l|}{2.40}     & 2.78 ± 0.34 & 1.72 ± 0.30       & 0.95 ± 0.39       & -44                                                                                  \\
PtrNet-RSA           & USNET             & 80                   & 320                                                               & 1.00    & \multicolumn{1}{l|}{2.80}     & 3.12 ± 0.33 & 2.05 ± 0.39      & 1.14 ± 0.40        & -14                                                                                     \\
PtrNet-RSA           & USNET             & 80                   & 330                                                               & 1.50  & \multicolumn{1}{l|}{3.10}     & 3.46 ± 0.34 & 2.34 ± 0.33      & 1.42 ± 0.46       & 5                                                                                   
\end{longtable}
\twocolumn


==> archive/truncation.tex <==




\subsection{Holding time truncation}
\label{sec:holding_time}

The traffic model in DeepRMSA and follow-up works includes an unusual detail: the service holding time is resampled if the resulting value is more than twice the mean of the inverse exponential PDF. We refer to this detail as holding time truncation. 


\subsubsection{Experiment setup}
To understand the effect of truncation on the traffic statistics, we define an inverse exponential PDF that is normalized to have unit mean. We take $10^{6}$ samples from the PDF, both with and without truncation, and calculate the mean of the resulting sample populations in both cases.

\subsubsection{Results and discussion}
Figure \ref{fig:truncation} compares histograms of service holding times with and without truncation. We define the bin width as 0.01 and normalize the count per bin to give a peak density of 1 without truncation. The truncated case shows a cutoff at twice the mean holding time. The vertical lines indicate the mean holding time for each case.

Holding time truncation reduces the mean by approximately 31\%. This results in 31\% lower traffic load. Therefore, papers that use the DeepRMSA codebase (including DeepRMSA, Reward-RMSA, and GCN-RMSA) evaluate their solutions at traffic loads 31\% lower than reported. This detail is not made explicit in the published papers. This finding highlights the challenges in making fair comparisons between papers, and the need for transparency in research code.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{IMAGES/truncation.png}
    \caption{Histogram of service holding holding times. The truncated distribution resamples the holding time when the sampled value exceeds 2*mean. This reduces the mean holding time by 31\% compared to the inverse exponential distribution.}
    \label{fig:truncation}
\end{figure}



%Cisco NCS 2000 Flex Spectrum Single Module ROADM and it's integrated pre-amplifier has a nominal noise figure of 5.5dB (for 24dB gain) or 11.7dB (for 12dB gain), 




==> archive/warmup.tex <==

\subsection{Network traffic warm-up}
\label{sec:warmup}

To exactly recreate the problem settings from the selected papers, it is necessary to generate the same number of traffic requests as the original work. This includes the connection requests that are generated to pre-populate the network until the blocking probability reaches steady-state, a phenomenon which is well-known in discrete-event simulation \cite{banks_discrete-event_2005}. We call the period prior to steady-state the warm-up period. 

Network warm-up is important so that the blocking probability reaches its steady-state value and is not an underestimate. This is known as the simulation start-up problem or the initial transient \cite{white_problem_2009}. During training, warm-up helps prevent primacy bias \cite{nikishin_primacy_2022}, where models overfit to data seen early in training. When starting with an empty network, initial traffic requests are trivially allocated due to abundant resources, providing no useful optimization signal. Training on a congested network with both successful and failed allocations gives more meaningful training data from the start.

While most papers do not explicitly discuss warm-up, all of the selected papers use it. We therefore analyze the minimum required warm-up period for different traffic levels.

\subsubsection{Experiment setup}

We simulate a non-blocking network to determine the maximum\footnotemark number of requests needed to reach a steady-state traffic load. For each traffic load from 50 to 1000 Erlangs in steps of 50, we conduct 500 simulation trials with unique random seeds at varying arrival rates from 5 to 25.  For each trial, we estimate the number of requests at which steady state is reached using the MSER-5 method \cite{franklin_stationarity_2008} (Marginal Standard Error Rule with batch size 5). We apply the MSER-5 method as it has been shown to be superior to other methods such as the mean crossing rule \cite{white_problem_2009}.


\footnotetext{A blocking network reaches steady-state in less steps than a non-blocking, therefore we consider a non-blocking network to estimate an upper bound on the required warm-up period before steady state.}


\subsubsection{Results and discussion}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{IMAGES/steady_state_boxplots.png}
    \caption{No. of simulated requests necessary to reach target network traffic level for a non-blocking network.}
    \label{fig:traffic_warmup}
\end{figure}

Figure \ref{fig:traffic_warmup} displays results as box-and-whisker plots showing how many requests are needed to reach steady state for each traffic load. The whiskers extend to the most extreme data points within 1.5 times the inter-quartile range. We observe a linear relationship between traffic load and requests until steady state (warm-up period). We fit a line to the maximum values (tops of the whiskers) to determine the warm-up period with high confidence. The fitted line indicates that approximately 7 times the target traffic load in requests are required to reach steady state. Based on this finding, the 3000-request warm-up period used by DeepRMSA that we adopt in section \ref{sec:repro} is sufficient for our problem settings.
